Multi-Fidelity Cost-Aware Bayesian Optimization

Bayesian optimization (BO) is increasingly employed in critical applications such as materials design and drug discovery. An increasingly popular strategy in BO is to forgo the sole reliance on high-fidelity data and instead use an ensemble of information sources which provide inexpensive low-fidelity data. The overall premise of this strategy is to reduce the overall sampling costs by querying inexpensive low-fidelity sources whose data are correlated with high-fidelity samples. Here, we propose a multi-fidelity cost-aware BO framework that dramatically outperforms the state-of-the-art technologies in terms of efficiency, consistency, and robustness. We demonstrate the advantages of our framework on analytic and engineering problems and argue that these benefits stem from our two main contributions: (1) we develop a novel acquisition function for multi-fidelity cost-aware BO that safeguards the convergence against the biases of low-fidelity data, and (2) we tailor a newly developed emulator for multi-fidelity BO which enables us to not only simultaneously learn from an ensemble of multi-fidelity datasets, but also identify the severely biased low-fidelity sources that should be excluded from BO.

==> 01_Ref.tex <==
@article{luong2021adaptive,
  title={Adaptive cost-aware Bayesian optimization},
  author={Luong, Phuc and Nguyen, Dang and Gupta, Sunil and Rana, Santu and Venkatesh, Svetha},
  journal={Knowledge-Based Systems},
  volume={232},
  pages={107481},
  year={2021},
  publisher={Elsevier}
}


@inproceedings{xu2020acquisition,
  title={Acquisition Function Selection: Bayesian Optimization in Neural Network Technique},
  author={Xu, Liuyang and Zhang, Zhongyue and Li, Zhengyang and Ke, Juntao},
  booktitle={2020 the 4th International Conference on Big Data Research (ICBDR'20)},
  pages={65--70},
  year={2020}
}

@article{frazier2018tutorial,
  title={A tutorial on Bayesian optimization},
  author={Frazier, Peter I},
  journal={arXiv preprint arXiv:1807.02811},
  year={2018}
}
@article{shahriari2015taking,
  title={Taking the human out of the loop: A review of Bayesian optimization},
  author={Shahriari, Bobak and Swersky, Kevin and Wang, Ziyu and Adams, Ryan P and De Freitas, Nando},
  journal={Proceedings of the IEEE},
  volume={104},
  number={1},
  pages={148--175},
  year={2015},
  publisher={IEEE}
}

@incollection{frazier2018bayesian,
  title={Bayesian optimization},
  author={Frazier, Peter I},
  booktitle={Recent advances in optimization and modeling of contemporary problems},
  pages={255--278},
  year={2018},
  publisher={Informs}
}

@inproceedings{li2004application,
  title={The application of Bayesian optimization and classifier systems in nurse scheduling},
  author={Li, Jingpeng and Aickelin, Uwe},
  booktitle={International Conference on Parallel Problem Solving from Nature},
  pages={581--590},
  year={2004},
  organization={Springer}
}

@article{sano2020application,
  title={Application of Bayesian optimization for pharmaceutical product development},
  author={Sano, Syusuke and Kadowaki, Tadashi and Tsuda, Koji and Kimura, Susumu},
  journal={Journal of Pharmaceutical Innovation},
  volume={15},
  number={3},
  pages={333--343},
  year={2020},
  publisher={Springer}
}

@article{huang2021bayesian,
  title={Bayesian optimization of functional output in inverse problems},
  author={Huang, Chaofan and Ren, Yi and McGuinness, Emily K and Losego, Mark D and Lively, Ryan P and Joseph, V Roshan},
  journal={Optimization and Engineering},
  volume={22},
  number={4},
  pages={2553--2574},
  year={2021},
  publisher={Springer}
}

@article{herbol2020cost,
  title={Cost-effective materials discovery: Bayesian optimization across multiple information sources},
  author={Herbol, Henry C and Poloczek, Matthias and Clancy, Paulette},
  journal={Materials Horizons},
  volume={7},
  number={8},
  pages={2113--2123},
  year={2020},
  publisher={Royal Society of Chemistry}
}

@article{cutajar2019deep,
  title={Deep gaussian processes for multi-fidelity modeling},
  author={Cutajar, Kurt and Pullin, Mark and Damianou, Andreas and Lawrence, Neil and Gonz{\'a}lez, Javier},
  journal={arXiv preprint arXiv:1903.07320},
  year={2019}
}

@article{meng2020composite,
  title={A composite neural network that learns from multi-fidelity data: Application to function approximation and inverse PDE problems},
  author={Meng, Xuhui and Karniadakis, George Em},
  journal={Journal of Computational Physics},
  volume={401},
  pages={109020},
  year={2020},
  publisher={Elsevier}
}

@article{kennedy2000predicting,
  title={Predicting the output from a complex computer code when fast approximations are available},
  author={Kennedy, Marc C and O'Hagan, Anthony},
  journal={Biometrika},
  volume={87},
  number={1},
  pages={1--13},
  year={2000},
  publisher={Oxford University Press}
}

@article{bakr2001introduction,
  title={An introduction to the space mapping technique},
  author={Bakr, Mohamed H and Bandler, John W and Madsen, Kaj and S{\o}ndergaard, Jacob},
  journal={Optimization and Engineering},
  volume={2},
  number={4},
  pages={369--384},
  year={2001},
  publisher={Springer}
}

@article{choi2009two,
  title={Two-level multifidelity design optimization studies for supersonic jets},
  author={Choi, Seongim and Alonso, Juan J and Kroo, Ilan M},
  journal={Journal of Aircraft},
  volume={46},
  number={3},
  pages={776--790},
  year={2009}
}

@article{poloczek2017multi,
  title={Multi-information source optimization},
  author={Poloczek, Matthias and Wang, Jialei and Frazier, Peter},
  journal={Advances in neural information processing systems},
  volume={30},
  year={2017}
}
@article{herbol2020cost,
  title={Cost-effective materials discovery: Bayesian optimization across multiple information sources},
  author={Herbol, Henry C and Poloczek, Matthias and Clancy, Paulette},
  journal={Materials Horizons},
  volume={7},
  number={8},
  pages={2113--2123},
  year={2020},
  publisher={Royal Society of Chemistry}
}

@article{balandat2020botorch,
  title={BoTorch: a framework for efficient Monte-Carlo Bayesian optimization},
  author={Balandat, Maximilian and Karrer, Brian and Jiang, Daniel and Daulton, Samuel and Letham, Ben and Wilson, Andrew G and Bakshy, Eytan},
  journal={Advances in neural information processing systems},
  volume={33},
  pages={21524--21538},
  year={2020}
}

@article{cheng2007performance,
  title={Performance studies on six heuristic global optimization methods in the location of critical slip surface},
  author={Cheng, Yung Ming and Li, L and Chi, SC},
  journal={Computers and Geotechnics},
  volume={34},
  number={6},
  pages={462--484},
  year={2007},
  publisher={Elsevier}
}

@article{deb2002fast,
  title={A fast and elitist multiobjective genetic algorithm: NSGA-II},
  author={Deb, Kalyanmoy and Pratap, Amrit and Agarwal, Sameer and Meyarivan, TAMT},
  journal={IEEE transactions on evolutionary computation},
  volume={6},
  number={2},
  pages={182--197},
  year={2002},
  publisher={IEEE}
}

@article{toal2011development,
  title={The development of a hybridized particle swarm for kriging hyperparameter tuning},
  author={Toal, David JJ and Bressloff, NW and Keane, AJ and Holden, CME},
  journal={Engineering optimization},
  volume={43},
  number={6},
  pages={675--699},
  year={2011},
  publisher={Taylor \& Francis}
}

@article{brochu2010tutorial,
  title={A tutorial on Bayesian optimization of expensive cost functions, with application to active user modeling and hierarchical reinforcement learning},
  author={Brochu, Eric and Cora, Vlad M and De Freitas, Nando},
  journal={arXiv preprint arXiv:1012.2599},
  year={2010}
}

@article{gelbart2014bayesian,
  title={Bayesian optimization with unknown constraints},
  author={Gelbart, Michael A and Snoek, Jasper and Adams, Ryan P},
  journal={arXiv preprint arXiv:1403.5607},
  year={2014}
}


@article{lizotte2008practical,
  title={Practical bayesian optimization},
  author={Lizotte, Daniel James},
  year={2008}
}

@inproceedings{wang2017new,
  title={A new acquisition function for Bayesian optimization based on the moment-generating function},
  author={Wang, Hao and van Stein, Bas and Emmerich, Michael and Back, Thomas},
  booktitle={2017 IEEE International Conference on Systems, Man, and Cybernetics (SMC)},
  pages={507--512},
  year={2017},
  organization={IEEE}
}
@article{srinivas2012information,
  title={Information-theoretic regret bounds for gaussian process optimization in the bandit setting},
  author={Srinivas, Niranjan and Krause, Andreas and Kakade, Sham M and Seeger, Matthias W},
  journal={IEEE transactions on information theory},
  volume={58},
  number={5},
  pages={3250--3265},
  year={2012},
  publisher={IEEE}
}

@phdthesis{wu2017knowledge,
  title={Knowledge Gradient Methods for Bayesian Optimization},
  author={Wu, Jian},
  year={2017},
  school={Cornell University}
}
@inproceedings{wang2017new,
  title={A new acquisition function for Bayesian optimization based on the moment-generating function},
  author={Wang, Hao and van Stein, Bas and Emmerich, Michael and Back, Thomas},
  booktitle={2017 IEEE International Conference on Systems, Man, and Cybernetics (SMC)},
  pages={507--512},
  year={2017},
  organization={IEEE}
}
@article{jones1998efficient,
  title={Efficient global optimization of expensive black-box functions},
  author={Jones, Donald R and Schonlau, Matthias and Welch, William J},
  journal={Journal of Global optimization},
  volume={13},
  number={4},
  pages={455--492},
  year={1998},
  publisher={Springer}
}

@article{jones2001taxonomy,
  title={A taxonomy of global optimization methods based on response surfaces},
  author={Jones, Donald R},
  journal={Journal of global optimization},
  volume={21},
  number={4},
  pages={345--383},
  year={2001},
  publisher={Springer}
}

@article{gutmann2001radial,
  title={A radial basis function method for global optimization},
  author={Gutmann, H-M},
  journal={Journal of global optimization},
  volume={19},
  number={3},
  pages={201--227},
  year={2001},
  publisher={Springer}
}

@article{jones1998efficient,
  title={Efficient global optimization of expensive black-box functions},
  author={Jones, Donald R and Schonlau, Matthias and Welch, William J},
  journal={Journal of Global optimization},
  volume={13},
  number={4},
  pages={455--492},
  year={1998},
  publisher={Springer}
}
@article{schonlau1998global,
  title={Global versus local search in constrained optimization of computer models},
  author={Schonlau, Matthias and Welch, William J and Jones, Donald R},
  journal={Lecture notes-monograph series},
  pages={11--25},
  year={1998},
  publisher={JSTOR}
}

@article{lyu2017efficient,
  title={An efficient bayesian optimization approach for automated optimization of analog circuits},
  author={Lyu, Wenlong and Xue, Pan and Yang, Fan and Yan, Changhao and Hong, Zhiliang and Zeng, Xuan and Zhou, Dian},
  journal={IEEE Transactions on Circuits and Systems I: Regular Papers},
  volume={65},
  number={6},
  pages={1954--1967},
  year={2017},
  publisher={IEEE}
}
@article{oune2021latent,
  title={Latent map Gaussian processes for mixed variable metamodeling},
  author={Oune, Nicholas and Bostanabad, Ramin},
  journal={Computer Methods in Applied Mechanics and Engineering},
  volume={387},
  pages={114128},
  year={2021},
  publisher={Elsevier}
}

@article{snoek2012practical,
  title={Practical bayesian optimization of machine learning algorithms},
  author={Snoek, Jasper and Larochelle, Hugo and Adams, Ryan P},
  journal={Advances in neural information processing systems},
  volume={25},
  year={2012}
}

@article{calandra2016bayesian,
  title={Bayesian optimization for learning gaits under uncertainty},
  author={Calandra, Roberto and Seyfarth, Andr{\'e} and Peters, Jan and Deisenroth, Marc Peter},
  journal={Annals of Mathematics and Artificial Intelligence},
  volume={76},
  number={1},
  pages={5--23},
  year={2016},
  publisher={Springer}
}

@article{roveda2021human,
  title={Human--robot collaboration in sensorless assembly task learning enhanced by uncertainties adaptation via Bayesian Optimization},
  author={Roveda, Loris and Magni, Mauro and Cantoni, Martina and Piga, Dario and Bucca, Giuseppe},
  journal={Robotics and Autonomous Systems},
  volume={136},
  pages={103711},
  year={2021},
  publisher={Elsevier}
}
@article{griffiths2020constrained,
  title={Constrained Bayesian optimization for automatic chemical design using variational autoencoders},
  author={Griffiths, Ryan-Rhys and Hern{\'a}ndez-Lobato, Jos{\'e} Miguel},
  journal={Chemical science},
  volume={11},
  number={2},
  pages={577--586},
  year={2020},
  publisher={Royal Society of Chemistry}
}

@article{ebikade2020active,
  title={Active learning-driven quantitative synthesis--structure--property relations for improving performance and revealing active sites of nitrogen-doped carbon for the hydrogen evolution reaction},
  author={Ebikade, Elvis Osamudiamhen and Wang, Yifan and Samulewicz, Nicholas and Hasa, Bjorn and Vlachos, Dionisios},
  journal={Reaction Chemistry \& Engineering},
  volume={5},
  number={12},
  pages={2134--2147},
  year={2020},
  publisher={Royal Society of Chemistry}
}

@article{burger2020mobile,
  title={A mobile robotic chemist},
  author={Burger, Benjamin and Maffettone, Phillip M and Gusev, Vladimir V and Aitchison, Catherine M and Bai, Yang and Wang, Xiaoyan and Li, Xiaobo and Alston, Ben M and Li, Buyi and Clowes, Rob and others},
  journal={Nature},
  volume={583},
  number={7815},
  pages={237--241},
  year={2020},
  publisher={Nature Publishing Group}
}

@article{tao2019input,
  title={Input mapping for model calibration with application to wing aerodynamics},
  author={Tao, Siyu and Apley, Daniel W and Chen, Wei and Garbo, Andrea and Pate, David J and German, Brian J},
  journal={AIAA journal},
  volume={57},
  number={7},
  pages={2734--2745},
  year={2019},
  publisher={American Institute of Aeronautics and Astronautics}
}
@article{bandler1994space,
  title={Space mapping technique for electromagnetic optimization},
  author={Bandler, John W and Biernacki, Radoslaw M and Chen, Shao Hua and Grobelny, Piotr A and Hemmers, Ronald H},
  journal={IEEE Transactions on microwave theory and techniques},
  volume={42},
  number={12},
  pages={2536--2544},
  year={1994},
  publisher={IEEE}
}

@article{li2017vf,
  title={A VF-SLP framework using least squares hybrid scaling for RBDO},
  author={Li, Xiaoke and Qiu, Haobo and Jiang, Zheng and Gao, Liang and Shao, Xinyu},
  journal={Structural and Multidisciplinary Optimization},
  volume={55},
  number={5},
  pages={1629--1640},
  year={2017},
  publisher={Springer}
}

@article{winter2022stochastic,
  title={Stochastic multi-fidelity surrogate modeling of dendritic crystal growth},
  author={Winter, JM and Kaiser, JWJ and Adami, S and Akhatov, IS and Adams, NA},
  journal={Computer Methods in Applied Mechanics and Engineering},
  volume={393},
  pages={114799},
  year={2022},
  publisher={Elsevier}
}

@book{sobester2008engineering,
  title={Engineering design via surrogate modelling: a practical guide},
  author={Sobester, Andr{\'a}s and Forrester, Alexander and Keane, Andy},
  year={2008},
  publisher={John Wiley \& Sons}
}
@article{perdikaris2016model,
  title={Model inversion via multi-fidelity Bayesian optimization: a new paradigm for parameter estimation in haemodynamics, and beyond},
  author={Perdikaris, Paris and Karniadakis, George Em},
  journal={Journal of The Royal Society Interface},
  volume={13},
  number={118},
  pages={20151107},
  year={2016},
  publisher={The Royal Society}
}
@article{perdikaris2016multifidelity,
  title={Multifidelity information fusion algorithms for high-dimensional systems and massive data sets},
  author={Perdikaris, Paris and Venturi, Daniele and Karniadakis, George Em},
  journal={SIAM Journal on Scientific Computing},
  volume={38},
  number={4},
  pages={B521--B538},
  year={2016},
  publisher={SIAM}
}
@article{perdikaris2017nonlinear,
  title={Nonlinear information fusion algorithms for data-efficient multi-fidelity modelling},
  author={Perdikaris, Paris and Raissi, Maziar and Damianou, Andreas and Lawrence, Neil D and Karniadakis, George Em},
  journal={Proceedings of the Royal Society A: Mathematical, Physical and Engineering Sciences},
  volume={473},
  number={2198},
  pages={20160751},
  year={2017},
  publisher={The Royal Society Publishing}
}

@inproceedings{song2019general,
  title={A general framework for multi-fidelity bayesian optimization with gaussian processes},
  author={Song, Jialin and Chen, Yuxin and Yue, Yisong},
  booktitle={The 22nd International Conference on Artificial Intelligence and Statistics},
  pages={3158--3167},
  year={2019},
  organization={PMLR}
}
@inproceedings{wu2020practical,
  title={Practical multi-fidelity Bayesian optimization for hyperparameter tuning},
  author={Wu, Jian and Toscano-Palmerin, Saul and Frazier, Peter I and Wilson, Andrew Gordon},
  booktitle={Uncertainty in Artificial Intelligence},
  pages={788--798},
  year={2020},
  organization={PMLR}
}
@inproceedings{zhu2020accelerating,
  title={Accelerating Hyperparameter Optimization of Deep Neural Network via Progressive Multi-Fidelity Evaluation},
  author={Zhu, Guanghui and Zhu, Ruancheng},
  booktitle={Pacific-Asia Conference on Knowledge Discovery and Data Mining},
  pages={752--763},
  year={2020},
  organization={Springer}
}
@article{lindauer2019boah,
  title={BOAH: A tool suite for multi-fidelity bayesian optimization \& analysis of hyperparameters},
  author={Lindauer, Marius and Eggensperger, Katharina and Feurer, Matthias and Biedenkapp, Andr{\'e} and Marben, Joshua and M{\"u}ller, Philipp and Hutter, Frank},
  journal={arXiv preprint arXiv:1908.06756},
  year={2019}
}
@article{cho2020basic,
  title={Basic enhancement strategies when using Bayesian optimization for hyperparameter tuning of deep neural networks},
  author={Cho, Hyunghun and Kim, Yongjin and Lee, Eunjung and Choi, Daeyoung and Lee, Yongjae and Rhee, Wonjong},
  journal={IEEE Access},
  volume={8},
  pages={52588--52608},
  year={2020},
  publisher={IEEE}
}
@article{phiboon2021experiment,
  title={Experiment and computation multi-fidelity multi-objective airfoil design optimization of fixed-wing UAV},
  author={Phiboon, Tharathep and Khankwa, Krittin and Petcharat, Nutchanan and Phoksombat, Nattaphon and Kanazaki, Masahiro and Kishi, Yuki and Bureerat, Sujin and Ariyarit, Atthaphon},
  journal={Journal of Mechanical Science and Technology},
  volume={35},
  number={9},
  pages={4065--4072},
  year={2021},
  publisher={Springer}
}
@article{sun2022correlated,
  title={Correlated multi-objective multi-fidelity optimization for HLS directives design},
  author={Sun, Qi and Chen, Tinghuan and Liu, Siting and Chen, Jianli and Yu, Hao and Yu, Bei},
  journal={ACM Transactions on Design Automation of Electronic Systems (TODAES)},
  volume={27},
  number={4},
  pages={1--27},
  year={2022},
  publisher={ACM New York, NY}
}
@inproceedings{belakaria2020multi,
  title={Multi-fidelity multi-objective Bayesian optimization: An output space entropy search approach},
  author={Belakaria, Syrine and Deshwal, Aryan and Doppa, Janardhan Rao},
  booktitle={Proceedings of the AAAI Conference on artificial intelligence},
  volume={34},
  number={06},
  pages={10035--10043},
  year={2020}
}
@book{dahlin2014approximate,
  title={Approximate inference in state space models with intractable likelihoods using Gaussian process optimisation},
  author={Dahlin, Johan and Sch{\"o}n, Thomas Bo and Villani, Mattias},
  year={2014}
}
@inproceedings{imani2019mfbo,
  title={MFBO-SSM: Multi-fidelity Bayesian optimization for fast inference in state-space models},
  author={Imani, Mahdi and Ghoreishi, Seyede Fatemeh and Allaire, Douglas and Braga-Neto, Ulisses M},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={33},
  number={01},
  pages={7858--7865},
  year={2019}
}
@article{li2020multi,
  title={Multi-fidelity Bayesian optimization via deep neural networks},
  author={Li, Shibo and Xing, Wei and Kirby, Robert and Zhe, Shandian},
  journal={Advances in Neural Information Processing Systems},
  volume={33},
  pages={8521--8531},
  year={2020}
}
@article{pang2017discovering,
  title={Discovering variable fractional orders of advection--dispersion equations from field data using multi-fidelity Bayesian optimization},
  author={Pang, Guofei and Perdikaris, Paris and Cai, Wei and Karniadakis, George Em},
  journal={Journal of Computational Physics},
  volume={348},
  pages={694--714},
  year={2017},
  publisher={Elsevier}
}

@article{frazier2008knowledge,
  title={A knowledge-gradient policy for sequential information collection},
  author={Frazier, Peter I and Powell, Warren B and Dayanik, Savas},
  journal={SIAM Journal on Control and Optimization},
  volume={47},
  number={5},
  pages={2410--2439},
  year={2008},
  publisher={SIAM}
}
@article{wang2016new,
  title={A new Bayesian approach to multi-response surface optimization integrating loss function with posterior probability},
  author={Wang, Jianjun and Ma, Yizhong and Ouyang, Linhan and Tu, Yiliu},
  journal={European Journal of Operational Research},
  volume={249},
  number={1},
  pages={231--237},
  year={2016},
  publisher={Elsevier}
}
@inproceedings{astudillo2019bayesian,
  title={Bayesian optimization of composite functions},
  author={Astudillo, Raul and Frazier, Peter},
  booktitle={International Conference on Machine Learning},
  pages={354--363},
  year={2019},
  organization={PMLR}
}
@article{gelbart2014bayesian,
  title={Bayesian optimization with unknown constraints},
  author={Gelbart, Michael A and Snoek, Jasper and Adams, Ryan P},
  journal={arXiv preprint arXiv:1403.5607},
  year={2014}
}

@article{wang2020parallel,
  title={Parallel Bayesian global optimization of expensive functions},
  author={Wang, Jialei and Clark, Scott C and Liu, Eric and Frazier, Peter I},
  journal={Operations Research},
  volume={68},
  number={6},
  pages={1850--1865},
  year={2020},
  publisher={INFORMS}
}
@article{knowles2006parego,
  title={ParEGO: A hybrid algorithm with on-line landscape approximation for expensive multiobjective optimization problems},
  author={Knowles, Joshua},
  journal={IEEE Transactions on Evolutionary Computation},
  volume={10},
  number={1},
  pages={50--66},
  year={2006},
  publisher={IEEE}
}
@inproceedings{ponweiser2008multiobjective,
  title={Multiobjective optimization on a limited budget of evaluations using model-assisted S-Metric selection},
  author={Ponweiser, Wolfgang and Wagner, Tobias and Biermann, Dirk and Vincze, Markus},
  booktitle={International Conference on Parallel Problem Solving from Nature},
  pages={784--794},
  year={2008},
  organization={Springer}}

@article{srinivas2009gaussian,
  title={Gaussian process optimization in the bandit setting: No regret and experimental design},
  author={Srinivas, Niranjan and Krause, Andreas and Kakade, Sham M and Seeger, Matthias},
  journal={arXiv preprint arXiv:0912.3995},
  year={2009}
}

@article{russo2014learning,
  title={Learning to optimize via posterior sampling},
  author={Russo, Daniel and Van Roy, Benjamin},
  journal={Mathematics of Operations Research},
  volume={39},
  number={4},
  pages={1221--1243},
  year={2014},
  publisher={INFORMS}
}
@article{hernandez2014predictive,
  title={Predictive entropy search for efficient global optimization of black-box functions},
  author={Hern{\'a}ndez-Lobato, Jos{\'e} Miguel and Hoffman, Matthew W and Ghahramani, Zoubin},
  journal={Advances in neural information processing systems},
  volume={27},
  year={2014}
}
@article{bonilla2007multi,
  title={Multi-task Gaussian process prediction},
  author={Bonilla, Edwin V and Chai, Kian and Williams, Christopher},
  journal={Advances in neural information processing systems},
  volume={20},
  year={2007}
}

@article{herbol2020cost,
  title={Cost-effective materials discovery: Bayesian optimization across multiple information sources},
  author={Herbol, Henry C and Poloczek, Matthias and Clancy, Paulette},
  journal={Materials Horizons},
  volume={7},
  number={8},
  pages={2113--2123},
  year={2020},
  publisher={Royal Society of Chemistry}
}
@inproceedings{matsubara2016data,
  title={Data-efficient human training of a care motion controller for human transfer assistant robots using bayesian optimization},
  author={Matsubara, Takamitsu and Funaki, Yoshihito and Ding, Ming and Ogasawara, Tsukasa and Sugimoto, Kenji},
  booktitle={2016 6th IEEE International Conference on Biomedical Robotics and Biomechatronics (BioRob)},
  pages={606--611},
  year={2016},
  organization={IEEE}
}
@article{bostanabad2018leveraging,
  title={Leveraging the nugget parameter for efficient Gaussian process modeling},
  author={Bostanabad, Ramin and Kearney, Tucker and Tao, Siyu and Apley, Daniel W and Chen, Wei},
  journal={International journal for numerical methods in engineering},
  volume={114},
  number={5},
  pages={501--516},
  year={2018},
  publisher={Wiley Online Library}
}
@inproceedings{ponweiser2008multiobjective,
  title={Multiobjective optimization on a limited budget of evaluations using model-assisted S-Metric selection},
  author={Ponweiser, Wolfgang and Wagner, Tobias and Biermann, Dirk and Vincze, Markus},
  booktitle={International Conference on Parallel Problem Solving from Nature},
  pages={784--794},
  year={2008},
  organization={Springer}
}
@article{zhang2020bayesian,
  title={Bayesian optimization for materials design with mixed quantitative and qualitative variables},
  author={Zhang, Yichi and Apley, Daniel W and Chen, Wei},
  journal={Scientific reports},
  volume={10},
  number={1},
  pages={1--13},
  year={2020},
  publisher={Nature Publishing Group}
}
@article{wu2019hyperparameter,
  title={Hyperparameter optimization for machine learning models based on Bayesian optimization},
  author={Wu, Jia and Chen, Xiu-Yun and Zhang, Hao and Xiong, Li-Dong and Lei, Hang and Deng, Si-Hao},
  journal={Journal of Electronic Science and Technology},
  volume={17},
  number={1},
  pages={26--40},
  year={2019},
  publisher={Elsevier}
}
@inproceedings{pautrat2018bayesian,
  title={Bayesian optimization with automatic prior selection for data-efficient direct policy search},
  author={Pautrat, R{\'e}mi and Chatzilygeroudis, Konstantinos and Mouret, Jean-Baptiste},
  booktitle={2018 IEEE International Conference on Robotics and Automation (ICRA)},
  pages={7571--7578},
  year={2018},
  organization={IEEE}
}
@article{shahriari2015taking,
  title={Taking the human out of the loop: A review of Bayesian optimization},
  author={Shahriari, Bobak and Swersky, Kevin and Wang, Ziyu and Adams, Ryan P and De Freitas, Nando},
  journal={Proceedings of the IEEE},
  volume={104},
  number={1},
  pages={148--175},
  year={2015},
  publisher={IEEE}
}

@article{zhang2021two,
  title={Two-step Lookahead Bayesian Optimization with Inequality Constraints},
  author={Zhang, Yunxiang and Zhang, Xiangyu and Frazier, Peter I},
  journal={arXiv preprint arXiv:2112.02833},
  year={2021}
}

@article{stainforth2005uncertainty,
  title={Uncertainty in predictions of the climate response to rising levels of greenhouse gases},
  author={Stainforth, David A and Aina, Tolu and Christensen, Carl and Collins, Mat and Faull, Nick and Frame, Dave J and Kettleborough, Jamie A and Knight, S and Martin, A and Murphy, JM and others},
  journal={Nature},
  volume={433},
  number={7024},
  pages={403--406},
  year={2005},
  publisher={Nature Publishing Group}
}
@article{zhang2019numerical,
  title={A numerical Bayesian-calibrated characterization method for multiscale prepreg preforming simulations with tension-shear coupling},
  author={Zhang, Weizhao and Bostanabad, Ramin and Liang, Biao and Su, Xuming and Zeng, Danielle and Bessa, Miguel A and Wang, Yanchao and Chen, Wei and Cao, Jian},
  journal={Composites Science and Technology},
  volume={170},
  pages={15--24},
  year={2019},
  publisher={Elsevier}
}
@article{yeom2019performance,
  title={Performance evaluation of automobile fuel consumption using a fuzzy-based granular model with coverage and specificity},
  author={Yeom, Chan-Uk and Kwak, Keun-Chang},
  journal={Symmetry},
  volume={11},
  number={12},
  pages={1480},
  year={2019},
  publisher={MDPI}
}


@article{RN412,
   author = {Ababou, Rachid and Bagtzoglou, Amvrossios C. and Wood, Eric F.},
   title = {On the condition number of covariance matrices in kriging, estimation, and simulation of random fields},
   journal = {Mathematical Geology},
   volume = {26},
   number = {1},
   pages = {99-133},
   ISSN = {0882-8121
1573-8868},
   DOI = {10.1007/bf02065878},
   url = {<Go to ISI>://WOS:A1994MU69900006},
   year = {1994},
   type = {Journal Article}
}

@article{RN1579,
   author = {Alvarez, Mauricio A. and Rosasco, Lorenzo and Lawrence, Neil D.},
   title = {Kernels for vector-valued functions: A review},
   journal = {arXiv preprint arXiv:1106.6251},
   year = {2011},
   type = {Journal Article}
}

@article{RN325,
   author = {Ankenman, Bruce and Nelson, Barry L. and Staum, Jeremy},
   title = {Stochastic Kriging for Simulation Metamodeling},
   journal = {Operations Research},
   volume = {58},
   number = {2},
   pages = {371-382},
   ISSN = {0030-364X
1526-5463},
   DOI = {10.1287/opre.1090.0754},
   url = {<Go to ISI>://WOS:000276735200009},
   year = {2010},
   type = {Journal Article}
}

@misc{RN1576,
   volume = {97},
   pages = {354--363},
   url = {https://proceedings.mlr.press/v97/astudillo19a.html},
   year = {2019},
   type = {Conference Paper}
}

@article{RN340,
   author = {Ba, Shan and Joseph, V. Roshan},
   title = {Composite Gaussian process models for emulating expensive functions},
   journal = {The Annals of Applied Statistics},
   volume = {6},
   number = {4},
   pages = {1838-1860},
   ISSN = {1932-6157},
   DOI = {10.1214/12-aoas570},
   url = {<Go to ISI>://WOS:000314458400021},
   year = {2012},
   type = {Journal Article}
}

@article{RN578,
   author = {Balachandran, P. V. and Xue, D. and Theiler, J. and Hogden, J. and Lookman, T.},
   title = {Adaptive Strategies for Materials Design using Uncertainties},
   journal = {Sci Rep},
   volume = {6},
   pages = {19660},
   ISSN = {2045-2322 (Electronic)
2045-2322 (Linking)},
   DOI = {10.1038/srep19660},
   url = {https://www.ncbi.nlm.nih.gov/pubmed/26792532},
   year = {2016},
   type = {Journal Article}
}

@article{RN1392,
   author = {Balandat, Maximilian and Karrer, Brian and Jiang, Daniel and Daulton, Samuel and Letham, Ben and Wilson, Andrew G. and Bakshy, Eytan},
   title = {BoTorch: A framework for efficient Monte-Carlo Bayesian optimization},
   journal = {Advances in Neural Information Processing Systems},
   volume = {33},
   year = {2020},
   type = {Journal Article}
}

@article{RN715,
   author = {Bastos, Leonardo S. and O’Hagan, Anthony},
   title = {Diagnostics for Gaussian Process Emulators},
   journal = {Technometrics},
   volume = {51},
   number = {4},
   pages = {425-438},
   ISSN = {0040-1706
1537-2723},
   DOI = {10.1198/tech.2009.08019},
   url = {<Go to ISI>://WOS:000272734100008},
   year = {2009},
   type = {Journal Article}
}

@article{RN687,
   author = {Ben-Ari, Einat Neumann and Steinberg, David M},
   title = {Modeling data from computer experiments: an empirical comparison of kriging with MARS and projection pursuit regression},
   journal = {Quality Engineering},
   volume = {19},
   number = {4},
   pages = {327-338},
   ISSN = {0898-2112},
   year = {2007},
   type = {Journal Article}
}

@article{RN318,
   author = {Bhat, Chandra R.},
   title = {Simulation estimation of mixed discrete choice models using randomized and scrambled Halton sequences},
   journal = {Transportation Research Part B: Methodological},
   volume = {37},
   number = {9},
   pages = {837-855},
   ISSN = {01912615},
   DOI = {10.1016/s0191-2615(02)00090-5},
   url = {<Go to ISI>://WOS:000184959900004},
   year = {2003},
   type = {Journal Article}
}

@article{RN530,
   author = {Bouhlel, Mohamed Amine and Martins, Joaquim RRA},
   title = {Gradient-enhanced kriging for high-dimensional problems},
   journal = {arXiv preprint arXiv:1708.02663},
   year = {2017},
   type = {Journal Article}
}

@article{RN689,
   author = {Chaloner, Kathryn and Verdinelli, Isabella},
   title = {Bayesian Experimental Design: A Review},
   journal = {Statistical Science},
   volume = {10},
   number = {3},
   pages = {273-304},
   ISSN = {0883-4237},
   DOI = {10.1214/ss/1177009939},
   url = {<Go to ISI>://WOS:A1995UN93700003},
   year = {1995},
   type = {Journal Article}
}

@article{RN615,
   author = {Chib, Siddhartha and Greenberg, Edward},
   title = {Understanding the Metropolis-Hastings Algorithm},
   journal = {The American Statistician},
   volume = {49},
   number = {4},
   pages = {327-335},
   ISSN = {00031305},
   DOI = {10.2307/2684568},
   url = {<Go to ISI>://WOS:A1995TK39900001},
   year = {1995},
   type = {Journal Article}
}

@article{RN316,
   author = {Chung, Hyoung-Seog and Alonso, Juan J},
   title = {Using gradients to construct cokriging approximation models for high-dimensional design optimization problems},
   journal = {AIAA paper},
   volume = {317},
   pages = {14-17},
   year = {2002},
   type = {Journal Article}
}

@article{RN675,
   author = {Constantine, Paul G. and Dow, Eric and Wang, Qiqi},
   title = {Active Subspace Methods in Theory and Practice: Applications to Kriging Surfaces},
   journal = {SIAM Journal on Scientific Computing},
   volume = {36},
   number = {4},
   pages = {A1500-A1524},
   ISSN = {1064-8275
1095-7197},
   DOI = {10.1137/130916138},
   url = {https://doi.org/10.1137/130916138},
   year = {2014},
   type = {Journal Article}
}

@article{RN328,
   author = {Conti, S. and Gosling, J. P. and Oakley, J. E. and O'Hagan, A.},
   title = {Gaussian process emulation of dynamic computer codes},
   journal = {Biometrika},
   volume = {96},
   number = {3},
   pages = {663-676},
   ISSN = {0006-3444
1464-3510},
   DOI = {10.1093/biomet/asp028},
   url = {<Go to ISI>://WOS:000269196300012},
   year = {2009},
   type = {Journal Article}
}

@article{RN287,
   author = {Conti, Stefano and O’Hagan, Anthony},
   title = {Bayesian emulation of complex multi-output and dynamic computer models},
   journal = {Journal of Statistical Planning and Inference},
   volume = {140},
   number = {3},
   pages = {640-651},
   ISSN = {03783758},
   DOI = {10.1016/j.jspi.2009.08.006},
   url = {<Go to ISI>://WOS:000272635800005},
   year = {2010},
   type = {Journal Article}
}

@inproceedings{RN378,
   author = {Crandell, Ian and Millican, Anthony J and Vasta, Robert and Smith, Eric and Alexander, Nathan and Devenport, William and Gramacy, Robert B and Binois, Mickaël},
   title = {Anomaly Detection in Large-Scale Wind Tunnel Tests Using Gaussian Processes},
   booktitle = {33rd AIAA Aerodynamic Measurement Technology and Ground Testing Conference},
   pages = {4131},
   type = {Conference Proceedings}
}

@article{RN302,
   author = {Cressie, Noel},
   title = {The origins of kriging},
   journal = {Mathematical Geology},
   volume = {22},
   number = {3},
   pages = {239-252},
   ISSN = {0882-8121
1573-8868},
   DOI = {10.1007/bf00889887},
   url = {<Go to ISI>://WOS:A1990CZ22300001},
   year = {1990},
   type = {Journal Article}
}

@article{RN474,
   author = {Cressie, Noel and Davidson, Jennifer L.},
   title = {Image analysis with partially ordered markov models},
   journal = {Computational Statistics & Data Analysis},
   volume = {29},
   number = {1},
   pages = {1-26},
   ISSN = {01679473},
   DOI = {10.1016/s0167-9473(98)00052-8},
   url = {<Go to ISI>://WOS:000077150200001},
   year = {1998},
   type = {Journal Article}
}

@article{RN299,
   author = {Cressie, Noel and Johannesson, Gardar},
   title = {Fixed rank kriging for very large spatial data sets},
   journal = {Journal of the Royal Statistical Society: Series B (Statistical Methodology)},
   volume = {70},
   number = {1},
   pages = {209-226},
   ISSN = {13697412},
   DOI = {10.1111/j.1467-9868.2007.00633.x},
   url = {<Go to ISI>://WOS:000252122500012},
   year = {2008},
   type = {Journal Article}
}

@article{RN1275,
   author = {Cutajar, Kurt and Pullin, Mark and Damianou, Andreas and Lawrence, Neil and González, Javier},
   title = {Deep gaussian processes for multi-fidelity modeling},
   journal = {arXiv preprint arXiv:1903.07320},
   year = {2019},
   type = {Journal Article}
}

@inproceedings{RN591,
   author = {Da Veiga, Sébastien and Marrel, Amandine},
   title = {Gaussian process modeling with inequality constraints},
   booktitle = {Annales de la Faculté des Sciences de Toulouse},
   volume = {21},
   pages = {529-555},
   type = {Conference Proceedings}
}

@inproceedings{RN718,
   author = {Damianou, Andreas and Lawrence, Neil},
   title = {Deep gaussian processes},
   booktitle = {Artificial Intelligence and Statistics},
   pages = {207-215},
   type = {Conference Proceedings}
}

@article{RN721,
   author = {Ding, Liang and Zhang, Xiaowei},
   title = {Scalable Stochastic Kriging with Markovian Covariances},
   journal = {arXiv preprint arXiv:1803.02575},
   year = {2018},
   type = {Journal Article}
}

@article{RN1426,
   author = {Du, Xianping and Xu, Hongyi and Zhu, Feng},
   title = {A data mining method for structure design with uncertainty in design variables},
   journal = {Computers & Structures},
   volume = {244},
   pages = {106457},
   ISSN = {0045-7949},
   year = {2021},
   type = {Journal Article}
}

@misc{RN895,
   pages = {467-478},
   year = {2018},
   type = {Conference Paper}
}

@article{RN900,
   author = {Feng, Chi and Marzouk, Youssef M},
   title = {A layered multiple importance sampling scheme for focused optimal Bayesian experimental design},
   journal = {arXiv preprint arXiv:1903.11187},
   year = {2019},
   type = {Journal Article}
}

@article{RN1587,
   author = {Figueiredo, Mario A. T. and Jain, Anil K.},
   title = {Unsupervised learning of finite mixture models},
   journal = {IEEE Transactions on pattern analysis and machine intelligence},
   volume = {24},
   number = {3},
   pages = {381-396},
   ISSN = {0162-8828},
   year = {2002},
   type = {Journal Article}
}

@article{RN1782,
   author = {Frazier, Peter and Powell, Warren and Dayanik, Savas},
   title = {The knowledge-gradient policy for correlated normal beliefs},
   journal = {INFORMS journal on Computing},
   volume = {21},
   number = {4},
   pages = {599-613},
   ISSN = {1091-9856},
   year = {2009},
   type = {Journal Article}
}

@article{RN1772,
   author = {Frazier, Peter I and Powell, Warren B and Dayanik, Savas},
   title = {A knowledge-gradient policy for sequential information collection},
   journal = {SIAM Journal on Control and Optimization},
   volume = {47},
   number = {5},
   pages = {2410-2439},
   ISSN = {0363-0129},
   year = {2008},
   type = {Journal Article}
}

@article{RN597,
   author = {Fricker, Thomas E. and Oakley, Jeremy E. and Urban, Nathan M.},
   title = {Multivariate Gaussian Process Emulators With Nonseparable Covariance Structures},
   journal = {Technometrics},
   volume = {55},
   number = {1},
   pages = {47-56},
   ISSN = {0040-1706
1537-2723},
   DOI = {10.1080/00401706.2012.715835},
   url = {<Go to ISI>://WOS:000321698000009},
   year = {2012},
   type = {Journal Article}
}

@article{RN294,
   author = {Furrer, R. and Genton, M. G. and Nychka, D.},
   title = {Erratum and Addendum to: “Covariance Tapering for Interpolation of Large Spatial Datasets” published in theJournal of Computational and Graphical Statistics, 15, 502–523},
   journal = {Journal of Computational and Graphical Statistics},
   volume = {21},
   number = {3},
   pages = {823-824},
   ISSN = {1061-8600
1537-2715},
   DOI = {10.1080/10618600.2012.712502},
   url = {<Go to ISI>://WOS:000308282000014},
   year = {2012},
   type = {Journal Article}
}

@inproceedings{RN671,
   author = {Garbo, Andrea and German, Brian},
   title = {Adaptive Sampling with Adaptive Surrogate Model Selection for Computer Experiment Applications},
   booktitle = {18th AIAA/ISSMO Multidisciplinary Analysis and Optimization Conference},
   pages = {4430},
   type = {Conference Proceedings}
}

@article{RN1270,
   author = {Gardner, Jacob R. and Pleiss, Geoff and Bindel, David and Weinberger, Kilian Q. and Wilson, Andrew Gordon},
   title = {Gpytorch: Blackbox matrix-matrix gaussian process inference with gpu acceleration},
   journal = {arXiv preprint arXiv:1809.11165},
   year = {2018},
   type = {Journal Article}
}

@article{RN1412,
   author = {Giovanis, Dimitris G. and Shields, Michael D.},
   title = {Data-driven surrogates for high dimensional models using Gaussian process regression on the Grassmann manifold},
   journal = {Computer Methods in Applied Mechanics and Engineering},
   volume = {370},
   pages = {113269},
   ISSN = {0045-7825},
   year = {2020},
   type = {Journal Article}
}

@article{RN1642,
   author = {Giselle Fernández-Godino, M and Park, Chanyoung and Kim, Nam H and Haftka, Raphael T},
   title = {Issues in deciding whether to use multifidelity surrogates},
   journal = {AIAA Journal},
   volume = {57},
   number = {5},
   pages = {2039-2054},
   ISSN = {0001-1452},
   year = {2019},
   type = {Journal Article}
}

@article{RN1770,
   author = {Gorodetsky, A. A. and Jakeman, J. D. and Geraci, G.},
   title = {MFNets: data efficient all-at-once learning of multifidelity surrogates as directed networks of information sources},
   journal = {Computational Mechanics},
   volume = {68},
   number = {4},
   pages = {741-758},
   ISSN = {1432-0924},
   DOI = {10.1007/s00466-021-02042-0},
   url = {https://doi.org/10.1007/s00466-021-02042-0},
   year = {2021},
   type = {Journal Article}
}

@article{RN503,
   author = {Gramacy, Robert B. and Apley, Daniel W.},
   title = {Local Gaussian Process Approximation for Large Computer Experiments},
   journal = {Journal of Computational and Graphical Statistics},
   volume = {24},
   number = {2},
   pages = {561-578},
   ISSN = {1061-8600
1537-2715},
   DOI = {10.1080/10618600.2014.914442},
   url = {<Go to ISI>://WOS:000356365700013},
   year = {2015},
   type = {Journal Article}
}

@article{RN380,
   author = {Gramacy, Robert B. and Haaland, Benjamin},
   title = {Speeding Up Neighborhood Search in Local Gaussian Process Prediction},
   journal = {Technometrics},
   volume = {58},
   number = {3},
   pages = {294-303},
   ISSN = {0040-1706
1537-2723},
   DOI = {10.1080/00401706.2015.1027067},
   url = {<Go to ISI>://WOS:000381014100003},
   year = {2016},
   type = {Journal Article}
}

@article{RN292,
   author = {Gramacy, Robert B. and Lee, Herbert K. H.},
   title = {Cases for the nugget in modeling computer experiments},
   journal = {Statistics and Computing},
   volume = {22},
   number = {3},
   pages = {713-722},
   ISSN = {0960-3174
1573-1375},
   DOI = {10.1007/s11222-010-9224-x},
   url = {<Go to ISI>://WOS:000302326400004},
   year = {2010},
   type = {Journal Article}
}

@article{RN347,
   author = {Gramacy, Robert B. and Lee, Herbert K. H.},
   title = {Bayesian Treed Gaussian Process Models With an Application to Computer Modeling},
   journal = {Journal of the American Statistical Association},
   volume = {103},
   number = {483},
   pages = {1119-1130},
   ISSN = {0162-1459
1537-274X},
   DOI = {10.1198/016214508000000689},
   url = {<Go to ISI>://WOS:000260193700018},
   year = {2012},
   type = {Journal Article}
}

@article{RN787,
   author = {Gramacy, Robert B. and Niemi, Jarad and Weiss, Robin M.},
   title = {Massively Parallel Approximate Gaussian Process Regression},
   journal = {SIAM/ASA Journal on Uncertainty Quantification},
   volume = {2},
   number = {1},
   pages = {564-584},
   ISSN = {2166-2525},
   DOI = {10.1137/130941912},
   url = {<Go to ISI>://WOS:000421346900024},
   year = {2014},
   type = {Journal Article}
}

@article{RN698,
   author = {Guhaniyogi, R. and Banerjee, S.},
   title = {Meta-Kriging: Scalable Bayesian Modeling and Inference for Massive Spatial Datasets},
   journal = {Technometrics},
   volume = {60},
   number = {4},
   pages = {430-444},
   ISSN = {0040-1706 (Print)
0040-1706 (Linking)},
   DOI = {10.1080/00401706.2018.1437474},
   url = {https://www.ncbi.nlm.nih.gov/pubmed/31007296},
   year = {2018},
   type = {Journal Article}
}

@article{RN322,
   author = {Han, Zhong-Hua and Görtz, Stefan and Zimmermann, Ralf},
   title = {Improving variable-fidelity surrogate modeling via gradient-enhanced kriging and a generalized hybrid bridge function},
   journal = {Aerospace Science and Technology},
   volume = {25},
   number = {1},
   pages = {177-189},
   ISSN = {12709638},
   DOI = {10.1016/j.ast.2012.01.006},
   url = {<Go to ISI>://WOS:000317442600019},
   year = {2013},
   type = {Journal Article}
}

@article{RN1221,
   author = {Harrow, A. W. and Hassidim, A. and Lloyd, S.},
   title = {Quantum algorithm for linear systems of equations},
   journal = {Phys Rev Lett},
   volume = {103},
   number = {15},
   pages = {150502},
   ISSN = {1079-7114 (Electronic)
0031-9007 (Linking)},
   DOI = {10.1103/PhysRevLett.103.150502},
   url = {https://www.ncbi.nlm.nih.gov/pubmed/19905613},
   year = {2009},
   type = {Journal Article}
}

@article{RN1722,
   author = {Hennig, Philipp and Schuler, Christian J},
   title = {Entropy Search for Information-Efficient Global Optimization},
   journal = {Journal of Machine Learning Research},
   volume = {13},
   number = {6},
   ISSN = {1532-4435},
   year = {2012},
   type = {Journal Article}
}

@article{RN893,
   author = {Hensman, James and Fusi, Nicolo and Lawrence, Neil D},
   title = {Gaussian processes for big data},
   journal = {arXiv preprint arXiv:1309.6835},
   year = {2013},
   type = {Journal Article}
}

@article{RN1569,
   author = {Hensman, James and Matthews, Alexander G. de G. and Filippone, Maurizio and Ghahramani, Zoubin},
   title = {MCMC for variationally sparse Gaussian processes},
   journal = {arXiv preprint arXiv:1506.04000},
   year = {2015},
   type = {Journal Article}
}

@article{RN1632,
   author = {Herbol, Henry C and Poloczek, Matthias and Clancy, Paulette},
   title = {Cost-effective materials discovery: Bayesian optimization across multiple information sources},
   journal = {Materials Horizons},
   volume = {7},
   number = {8},
   pages = {2113-2123},
   year = {2020},
   type = {Journal Article}
}

@inproceedings{RN1645,
   author = {Izmailov, Pavel and Vikram, Sharad and Hoffman, Matthew D and Wilson, Andrew Gordon Gordon},
   title = {What are Bayesian neural network posteriors really like?},
   booktitle = {International Conference on Machine Learning},
   publisher = {PMLR},
   pages = {4629-4640},
   ISBN = {2640-3498},
   type = {Conference Proceedings}
}

@article{RN449,
   author = {Jin, Ruichen and Chen, Wei and Sudjianto, Agus},
   title = {An efficient algorithm for constructing optimal design of computer experiments},
   journal = {Journal of Statistical Planning and Inference},
   volume = {134},
   number = {1},
   pages = {268-287},
   ISSN = {03783758},
   DOI = {10.1016/j.jspi.2004.02.014},
   url = {<Go to ISI>://WOS:000230058100018},
   year = {2005},
   type = {Journal Article}
}

@article{RN390,
   author = {Joseph, V. Roshan},
   title = {Limit Kriging},
   journal = {Technometrics},
   volume = {48},
   number = {4},
   pages = {458-466},
   ISSN = {0040-1706
1537-2723},
   DOI = {10.1198/004017006000000011},
   url = {<Go to ISI>://WOS:000242154100001},
   year = {2006},
   type = {Journal Article}
}

@article{RN273,
   author = {Kennedy, M.},
   title = {Predicting the output from a complex computer code when fast approximations are available},
   journal = {Biometrika},
   volume = {87},
   number = {1},
   pages = {1-13},
   ISSN = {0006-3444
1464-3510},
   DOI = {10.1093/biomet/87.1.1},
   url = {<Go to ISI>://WOS:000086307400001},
   year = {2000},
   type = {Journal Article}
}

@article{RN435,
   author = {Kim, Hyoung-Moon and Mallick, Bani K. and Holmes, C. C.},
   title = {Analyzing Nonstationary Spatial Data Using Piecewise Gaussian Processes},
   journal = {Journal of the American Statistical Association},
   volume = {100},
   number = {470},
   pages = {653-668},
   ISSN = {0162-1459
1537-274X},
   DOI = {10.1198/016214504000002014},
   url = {<Go to ISI>://WOS:000233311300026},
   year = {2005},
   type = {Journal Article}
}

@article{RN320,
   author = {Kleijnen, Jack P. C. and van Beers, Wim C. M.},
   title = {Robustness of Kriging when interpolating in random simulation with heterogeneous variances: Some experiments},
   journal = {European Journal of Operational Research},
   volume = {165},
   number = {3},
   pages = {826-834},
   ISSN = {03772217},
   DOI = {10.1016/j.ejor.2003.09.037},
   url = {<Go to ISI>://WOS:000228123800020},
   year = {2005},
   type = {Journal Article}
}

@article{RN807,
   author = {Knap, J. and Barton, N. R. and Hornung, R. D. and Arsenlis, A. and Becker, R. and Jefferson, D. R.},
   title = {Adaptive sampling in hierarchical simulation},
   journal = {International Journal for Numerical Methods in Engineering},
   volume = {76},
   number = {4},
   pages = {572-600},
   ISSN = {00295981
10970207},
   DOI = {10.1002/nme.2339},
   url = {<Go to ISI>://WOS:000260351400007},
   year = {2008},
   type = {Journal Article}
}

@article{RN1242,
   author = {Kusne, A. G. and Yu, H. and Wu, C. and Zhang, H. and Hattrick-Simpers, J. and DeCost, B. and Sarker, S. and Oses, C. and Toher, C. and Curtarolo, S. and Davydov, A. V. and Agarwal, R. and Bendersky, L. A. and Li, M. and Mehta, A. and Takeuchi, I.},
   title = {On-the-fly closed-loop materials discovery via Bayesian active learning},
   journal = {Nat Commun},
   volume = {11},
   number = {1},
   pages = {5966},
   ISSN = {2041-1723 (Electronic)
2041-1723 (Linking)},
   DOI = {10.1038/s41467-020-19597-w},
   url = {https://www.ncbi.nlm.nih.gov/pubmed/33235197},
   year = {2020},
   type = {Journal Article}
}

@inproceedings{RN1608,
   author = {Lalchand, Vidhi and Rasmussen, Carl Edward},
   title = {Approximate inference for fully Bayesian Gaussian process regression},
   booktitle = {Symposium on Advances in Approximate Bayesian Inference},
   publisher = {PMLR},
   pages = {1-12},
   ISBN = {2640-3498},
   type = {Conference Proceedings}
}

@inproceedings{RN1723,
   author = {Lam, Rémi and Allaire, Douglas L and Willcox, Karen E},
   title = {Multifidelity optimization using statistical surrogate modeling for non-hierarchical information sources},
   booktitle = {56th AIAA/ASCE/AHS/ASC Structures, Structural Dynamics, and Materials Conference},
   pages = {0143},
   type = {Conference Proceedings}
}

@article{RN1616,
   author = {Lam, Remi and Willcox, Karen},
   title = {Lookahead Bayesian optimization with inequality constraints},
   journal = {Advances in Neural Information Processing Systems},
   volume = {30},
   year = {2017},
   type = {Journal Article}
}

@article{RN729,
   author = {Lataniotis, Christos and Marelli, Stefano and Sudret, Bruno},
   title = {The Gaussian process modelling module in UQLab},
   journal = {Soft Computing in Civil Engineering},
   volume = {2},
   number = {3},
   pages = {91-116},
   DOI = {10.22115/scce.2018.129323.1062},
   url = {http://www.jsoftcivil.com/article_64721_329effd7ea1841207cec9b59c663ba5c.pdf},
   year = {2018},
   type = {Journal Article}
}

@article{RN291,
   author = {Laurenceau, J. and Sagaut, P.},
   title = {Building Efficient Response Surfaces of Aerodynamic Functions with Kriging and Cokriging},
   journal = {AIAA Journal},
   volume = {46},
   number = {2},
   pages = {498-507},
   ISSN = {0001-1452
1533-385X},
   DOI = {10.2514/1.32308},
   url = {<Go to ISI>://WOS:000252822800020},
   year = {2008},
   type = {Journal Article}
}

@inproceedings{RN717,
   author = {Le, Quoc V and Smola, Alex J and Canu, Stéphane},
   title = {Heteroscedastic Gaussian process regression},
   booktitle = {Proceedings of the 22nd international conference on Machine learning},
   publisher = {ACM},
   pages = {489-496},
   ISBN = {1595931805},
   type = {Conference Proceedings}
}

@article{RN837,
   author = {Lee, Seungjoon and Dietrich, Felix and Karniadakis, George E and Kevrekidis, Ioannis G},
   title = {Linking Gaussian Process regression with data-driven manifold embeddings for nonlinear data fusion},
   journal = {arXiv preprint arXiv:1812.06467},
   year = {2018},
   type = {Journal Article}
}

@article{RN289,
   author = {Li, G. and Azarm, S. and Farhang-Mehr, A. and Diaz, A. R.},
   title = {Approximation of multiresponse deterministic engineering simulations: a dependent metamodeling approach},
   journal = {Structural and Multidisciplinary Optimization},
   volume = {31},
   number = {4},
   pages = {260-269},
   ISSN = {1615-147X
1615-1488},
   DOI = {10.1007/s00158-005-0574-5},
   url = {<Go to ISI>://WOS:000236002400002},
   year = {2006},
   type = {Journal Article}
}

@article{RN1574,
   author = {Liu, H. and Ong, Y. S. and Shen, X. and Cai, J.},
   title = {When Gaussian Process Meets Big Data: A Review of Scalable GPs},
   journal = {IEEE Transactions on Neural Networks and Learning Systems},
   volume = {31},
   number = {11},
   pages = {4405-4423},
   ISSN = {2162-2388},
   DOI = {10.1109/TNNLS.2019.2957109},
   year = {2020},
   type = {Journal Article}
}

@article{RN319,
   author = {MacDonald, B. and Ranjan, P. and Chipman, H.},
   title = {GPfit: An R Package for Fitting a Gaussian Process Model to Deterministic Simulator Outputs},
   journal = {Journal of Statistical Software},
   volume = {64},
   number = {12},
   pages = {1-23},
   ISSN = {1548-7660},
   url = {<Go to ISI>://WOS:000352916200001},
   year = {2015},
   type = {Journal Article}
}

@article{RN1771,
   author = {Maddox, Wesley J and Balandat, Maximilian and Wilson, Andrew G and Bakshy, Eytan},
   title = {Bayesian optimization with high-dimensional outputs},
   journal = {Advances in Neural Information Processing Systems},
   volume = {34},
   pages = {19274-19287},
   year = {2021},
   type = {Journal Article}
}

@article{RN303,
   author = {Martin, Jay D. and Simpson, Timothy W.},
   title = {Use of Kriging Models to Approximate Deterministic Computer Models},
   journal = {AIAA Journal},
   volume = {43},
   number = {4},
   pages = {853-863},
   ISSN = {0001-1452
1533-385X},
   DOI = {10.2514/1.8650},
   url = {<Go to ISI>://WOS:000228246900016},
   year = {2005},
   type = {Journal Article}
}

@article{RN856,
   author = {Marzouk, Youssef and Moselhy, Tarek and Parno, Matthew and Spantini, Alessio},
   title = {An introduction to sampling via measure transport},
   journal = {arXiv preprint arXiv:1602.05023},
   year = {2016},
   type = {Journal Article}
}

@inproceedings{RN714,
   author = {McHutchon, Andrew and Rasmussen, Carl E},
   title = {Gaussian process training with input noise},
   booktitle = {Advances in Neural Information Processing Systems},
   pages = {1341-1349},
   type = {Conference Proceedings}
}

@article{RN326,
   author = {Meckesheimer, Martin and Barton, Russell R. and Simpson, Timothy and Limayem, Frej and Yannou, Bernard},
   title = {Metamodeling of Combined Discrete/Continuous Responses},
   journal = {AIAA Journal},
   volume = {39},
   number = {10},
   pages = {1950-1959},
   ISSN = {0001-1452
1533-385X},
   DOI = {10.2514/2.1185},
   url = {<Go to ISI>://WOS:000171445200015},
   year = {2001},
   type = {Journal Article}
}

@inproceedings{RN1062,
   author = {Mobahi, Hossein and Fisher III, John W},
   title = {A theoretical analysis of optimization by Gaussian continuation},
   booktitle = {Twenty-Ninth AAAI Conference on Artificial Intelligence},
   type = {Conference Proceedings}
}

@article{RN849,
   author = {Mohammadi-Ghazi, Reza and Marzouk, Youssef M. and Büyüköztürk, Oral},
   title = {Conditional classifiers and boosted conditional Gaussian mixture model for novelty detection},
   journal = {Pattern Recognition},
   volume = {81},
   pages = {601-614},
   ISSN = {00313203},
   DOI = {10.1016/j.patcog.2018.03.022},
   url = {<Go to ISI>://WOS:000436350700044},
   year = {2018},
   type = {Journal Article}
}

@article{RN857,
   author = {O'Hagan, A.},
   title = {Bayes–Hermite quadrature},
   journal = {Journal of Statistical Planning and Inference},
   volume = {29},
   number = {3},
   pages = {245-260},
   ISSN = {03783758},
   DOI = {10.1016/0378-3758(91)90002-v},
   url = {http://www.sciencedirect.com/science/article/pii/037837589190002V},
   year = {1991},
   type = {Journal Article}
}

@article{RN838,
   author = {Pang, Guofei and Yang, Liu and Karniadakis, George Em},
   title = {Neural-net-induced Gaussian process regression for function approximation and PDE solution},
   journal = {Journal of Computational Physics},
   volume = {384},
   pages = {270-288},
   ISSN = {00219991},
   DOI = {10.1016/j.jcp.2019.01.045},
   url = {<Go to ISI>://WOS:000460888400015},
   year = {2019},
   type = {Journal Article}
}

@article{RN818,
   author = {Park, C. and Apley, D.},
   title = {Patchwork Kriging for Large-scale Gaussian Process Regression},
   journal = {Journal of Machine Learning Research},
   volume = {19},
   number = {1},
   pages = {269-311},
   ISSN = {1532-4435},
   url = {<Go to ISI>://WOS:000443222900001},
   year = {2018},
   type = {Journal Article}
}

@article{RN338,
   author = {Paulo, Rui},
   title = {Default priors for Gaussian processes},
   journal = {The Annals of Statistics},
   volume = {33},
   number = {2},
   pages = {556-582},
   ISSN = {0090-5364},
   DOI = {10.1214/009053604000001264},
   url = {<Go to ISI>://WOS:000229853900005},
   year = {2005},
   type = {Journal Article}
}

@article{RN855,
   author = {Peherstorfer, Benjamin and Willcox, Karen},
   title = {Dynamic data-driven reduced-order models},
   journal = {Computer Methods in Applied Mechanics and Engineering},
   volume = {291},
   pages = {21-41},
   ISSN = {00457825},
   DOI = {10.1016/j.cma.2015.03.018},
   url = {<Go to ISI>://WOS:000354403300002},
   year = {2015},
   type = {Journal Article}
}

@article{RN1759,
   author = {Peng, Jiayu and Damewood, James K. and Karaguesian, Jessica and Gómez-Bombarelli, Rafael and Shao-Horn, Yang},
   title = {Navigating multimetallic catalyst space with Bayesian optimization},
   journal = {Joule},
   volume = {5},
   number = {12},
   pages = {3069-3071},
   ISSN = {2542-4351},
   DOI = {https://doi.org/10.1016/j.joule.2021.11.011},
   url = {https://www.sciencedirect.com/science/article/pii/S2542435121005377},
   year = {2021},
   type = {Journal Article}
}

@article{RN434,
   author = {Plumlee, Matthew and Apley, Daniel W.},
   title = {Lifted Brownian Kriging Models},
   journal = {Technometrics},
   volume = {59},
   number = {2},
   pages = {165-177},
   ISSN = {0040-1706
1537-2723},
   DOI = {10.1080/00401706.2016.1211555},
   url = {<Go to ISI>://WOS:000399588600003},
   year = {2017},
   type = {Journal Article}
}

@article{RN1405,
   author = {Plumlee, M. and Erickson, C. B. and Ankenman, B. E. and Lawrence, E.},
   title = {Composite grid designs for adaptive computer experiments with fast inference},
   journal = {Biometrika},
   year = {2020},
   type = {Journal Article}
}

@article{RN1631,
   author = {Poloczek, Matthias and Wang, Jialei and Frazier, Peter},
   title = {Multi-information source optimization},
   journal = {Advances in neural information processing systems},
   volume = {30},
   year = {2017},
   type = {Journal Article}
}

@article{RN1492,
   author = {Qian, Peter Z. G. and Wu, Huaiqing and Wu, C. F. Jeff},
   title = {Gaussian process models for computer experiments with qualitative and quantitative factors},
   journal = {Technometrics},
   volume = {50},
   number = {3},
   pages = {383-396},
   ISSN = {0040-1706},
   year = {2008},
   type = {Journal Article}
}

@article{RN892,
   author = {Raissi, Maziar},
   title = {Parametric Gaussian process regression for big data},
   journal = {arXiv preprint arXiv:1704.03144},
   year = {2017},
   type = {Journal Article}
}

@article{RN834,
   author = {Raissi, Maziar and Perdikaris, Paris and Karniadakis, George Em},
   title = {Machine learning of linear differential equations using Gaussian processes},
   journal = {Journal of Computational Physics},
   volume = {348},
   pages = {683-693},
   ISSN = {00219991},
   DOI = {10.1016/j.jcp.2017.07.050},
   url = {<Go to ISI>://WOS:000410899200033},
   year = {2017},
   type = {Journal Article}
}

@article{RN286,
   author = {Ranjan, Pritam and Haynes, Ronald and Karsten, Richard},
   title = {A Computationally Stable Approach to Gaussian Process Interpolation of Deterministic Computer Simulation Data},
   journal = {Technometrics},
   volume = {53},
   number = {4},
   pages = {366-378},
   ISSN = {0040-1706
1537-2723},
   DOI = {10.1198/tech.2011.09141},
   url = {<Go to ISI>://WOS:000297904600004},
   year = {2011},
   type = {Journal Article}
}

@inbook{RN1585,
   author = {Rasmussen, Carl Edward},
   title = {The Infinite Gaussian Mixture Model},
   booktitle = {Advances in information processing systems 12},
   publisher = {MIT Press},
   pages = {554-560},
   year = {2000},
   type = {Book Section}
}

@book{RN332,
   author = {Rasmussen, Carl Edward},
   title = {Gaussian processes for machine learning},
   year = {2006},
   type = {Book}
}

@inproceedings{RN816,
   author = {Rasmussen, Carl Edward and Quinonero-Candela, Joaquin},
   title = {Healing the relevance vector machine through augmentation},
   booktitle = {Proceedings of the 22nd international conference on Machine learning},
   publisher = {ACM},
   pages = {689-696},
   ISBN = {1595931805},
   type = {Conference Proceedings}
}

@inproceedings{RN1505,
   author = {Reece, Steven and Roberts, Stephen},
   title = {An introduction to Gaussian processes for the Kalman filter expert},
   booktitle = {2010 13th International Conference on Information Fusion},
   publisher = {IEEE},
   pages = {1-9},
   ISBN = {0982443811},
   type = {Conference Proceedings}
}

@inbook{RN1779,
   author = {Renganathan, Ashwin and Rao, Vishwas and Navon, Ionel},
   title = {Multifidelity Gaussian processes for failure boundary and probability estimation},
   booktitle = {AIAA SCITECH 2022 Forum},
   DOI = {10.2514/6.2022-0390},
   url = {https://arc.aiaa.org/doi/abs/10.2514/6.2022-0390},
   type = {Book Section}
}

@inproceedings{RN1396,
   author = {Rezende, Danilo Jimenez and Mohamed, Shakir and Wierstra, Daan},
   title = {Stochastic backpropagation and variational inference in deep latent gaussian models},
   publisher = {Citeseer},
   volume = {2},
   pages = {2},
   type = {Conference Proceedings}
}

@inproceedings{RN650,
   author = {Riihimäki, Jaakko and Vehtari, Aki},
   title = {Gaussian processes with monotonicity information},
   booktitle = {Proceedings of the Thirteenth International Conference on Artificial Intelligence and Statistics},
   pages = {645-652},
   type = {Conference Proceedings}
}

@article{RN283,
   author = {Roustant, O. and Ginsbourger, D. and Deville, Y.},
   title = {DiceKriging, DiceOptim: Two R Packages for the Analysis of Computer Experiments by Kriging-Based Metamodeling and Optimization},
   journal = {Journal of Statistical Software},
   volume = {51},
   number = {1},
   pages = {1-55},
   ISSN = {1548-7660},
   url = {<Go to ISI>://WOS:000310773900001},
   year = {2012},
   type = {Journal Article}
}

@article{RN1214,
   author = {Roustant, Olivier and Padonou, Esperan and Deville, Yves and Clément, Aloïs and Perrin, Guillaume and Giorla, Jean and Wynn, Henry},
   title = {Group kernels for Gaussian process metamodels with categorical inputs},
   journal = {SIAM/ASA Journal on Uncertainty Quantification},
   volume = {8},
   number = {2},
   pages = {775-806},
   ISSN = {2166-2525},
   year = {2020},
   type = {Journal Article}
}

@article{RN676,
   author = {Sacks, Jerome and Schiller, Susannah B. and Welch, William J.},
   title = {Designs for Computer Experiments},
   journal = {Technometrics},
   volume = {31},
   number = {1},
   pages = {41-47},
   ISSN = {00401706},
   DOI = {10.2307/1270363},
   url = {<Go to ISI>://WOS:A1989T692700005},
   year = {1989},
   type = {Journal Article}
}

@inproceedings{RN323,
   author = {Salemi, Peter and Staum, Jeremy and Nelson, Barry L},
   title = {Generalized integrated brownian fields for simulation metamodeling},
   booktitle = {Proceedings of the 2013 Winter Simulation Conference: Simulation: Making Decisions in a Complex World},
   publisher = {IEEE Press},
   pages = {543-554},
   ISBN = {1479920770},
   type = {Conference Proceedings}
}

@inbook{RN590,
   author = {Sanz-Serna, JM},
   title = {Markov chain Monte Carlo and numerical differential equations},
   booktitle = {Current challenges in stability issues for numerical differential equations},
   publisher = {Springer},
   pages = {39-88},
   year = {2014},
   type = {Book Section}
}

@article{RN1255,
   author = {Shan, Songqing and Wang, G. Gary},
   title = {Metamodeling for high dimensional simulation-based design problems},
   journal = {Journal of Mechanical Design},
   volume = {132},
   number = {5},
   ISSN = {1050-0472},
   year = {2010},
   type = {Journal Article}
}

@article{RN297,
   author = {Simpson, T. W. and Poplinski, J. D. and Koch, P. N. and Allen, J. K.},
   title = {Metamodels for Computer-based Engineering Design: Survey and recommendations},
   journal = {Engineering with Computers},
   volume = {17},
   number = {2},
   pages = {129-150},
   ISSN = {0177-0667
1435-5663},
   DOI = {10.1007/pl00007198},
   url = {<Go to ISI>://WOS:000170149900004},
   year = {2014},
   type = {Journal Article}
}

@inproceedings{RN1721,
   author = {Snoek, Jasper and Rippel, Oren and Swersky, Kevin and Kiros, Ryan and Satish, Nadathur and Sundaram, Narayanan and Patwary, Mostofa and Prabhat, Mr and Adams, Ryan},
   title = {Scalable bayesian optimization using deep neural networks},
   booktitle = {International conference on machine learning},
   publisher = {PMLR},
   pages = {2171-2180},
   type = {Conference Proceedings}
}

@article{RN114,
   author = {Sobol, I. M.},
   title = {On quasi-Monte Carlo integrations},
   journal = {Mathematics and Computers in Simulation},
   volume = {47},
   number = {2-5},
   pages = {103-112},
   ISSN = {03784754},
   DOI = {10.1016/s0378-4754(98)00096-2},
   url = {<Go to ISI>://WOS:000075073900003},
   year = {1998},
   type = {Journal Article}
}

@article{RN71,
   author = {Sobol', Il'ya Meerovich},
   title = {On the distribution of points in a cube and the approximate evaluation of integrals},
   journal = {Zhurnal Vychislitel'noi Matematiki i Matematicheskoi Fiziki},
   volume = {7},
   number = {4},
   pages = {784-802},
   ISSN = {0044-4669},
   year = {1967},
   type = {Journal Article}
}

@misc{RN1479,
   volume = {130},
   pages = {3133--3141},
   url = {http://proceedings.mlr.press/v130/stanton21a.html},
   year = {2021},
   type = {Conference Paper}
}

@book{RN301,
   author = {Stein, Michael L},
   title = {Interpolation of spatial data: some theory for kriging},
   publisher = {Springer Science & Business Media},
   ISBN = {1461214947},
   year = {2012},
   type = {Book}
}

@article{RN891,
   author = {Stuart, Andrew M. and Teckentrup, Aretha L.},
   title = {Posterior consistency for Gaussian process approximations of Bayesian posterior distributions},
   journal = {Mathematics of Computation},
   volume = {87},
   number = {310},
   pages = {721-753},
   ISSN = {0025-5718
1088-6842},
   DOI = {10.1090/mcom/3244},
   url = {<Go to ISI>://WOS:000418689600007},
   year = {2017},
   type = {Journal Article}
}

@article{RN1172,
   author = {Susiluoto, Jouni and Spantini, Alessio and Haario, Heikki and Härkönen, Teemu and Marzouk, Youssef},
   title = {Efficient multi-scale Gaussian process regression for massive remote sensing data with satGP v0.1.2},
   journal = {Geoscientific Model Development},
   volume = {13},
   number = {7},
   pages = {3439-3463},
   ISSN = {1991-9603},
   DOI = {10.5194/gmd-13-3439-2020},
   url = {<Go to ISI>://WOS:000558641100001},
   year = {2020},
   type = {Journal Article}
}

@article{RN1720,
   author = {Swersky, Kevin and Snoek, Jasper and Adams, Ryan P},
   title = {Multi-task bayesian optimization},
   journal = {Advances in neural information processing systems},
   volume = {26},
   year = {2013},
   type = {Journal Article}
}

@article{RN1640,
   author = {Swersky, Kevin and Snoek, Jasper and Adams, Ryan Prescott},
   title = {Freeze-thaw Bayesian optimization},
   journal = {arXiv preprint arXiv:1406.3896},
   year = {2014},
   type = {Journal Article}
}

@article{RN1134,
   author = {Tao, Siyu and Apley, Daniel W. and Chen, Wei and Garbo, Andrea and Pate, David J. and German, Brian J.},
   title = {Input Mapping for Model Calibration with Application to Wing Aerodynamics},
   journal = {AIAA Journal},
   volume = {57},
   number = {7},
   pages = {2734-2745},
   ISSN = {0001-1452
1533-385X},
   DOI = {10.2514/1.J057711},
   url = {<Go to ISI>://WOS:000488793600008},
   year = {2019},
   type = {Journal Article}
}

@article{RN1586,
   author = {Teh, Yee Whye and Jordan, Michael I. and Beal, Matthew J. and Blei, David M.},
   title = {Hierarchical Dirichlet Processes},
   journal = {Journal of the American Statistical Association},
   volume = {101},
   number = {476},
   pages = {1566-1581},
   ISSN = {0162-1459},
   DOI = {10.1198/016214506000000302},
   url = {https://doi.org/10.1198/016214506000000302},
   year = {2006},
   type = {Journal Article}
}

@article{RN713,
   author = {Thimmisetty, Charanraj A. and Ghanem, Roger G. and White, Joshua A. and Chen, Xiao},
   title = {High-Dimensional Intrinsic Interpolation Using Gaussian Process Regression and Diffusion Maps},
   journal = {Mathematical Geosciences},
   volume = {50},
   number = {1},
   pages = {77-96},
   ISSN = {1874-8961
1874-8953},
   DOI = {10.1007/s11004-017-9705-y},
   url = {<Go to ISI>://WOS:000419166200004},
   year = {2017},
   type = {Journal Article}
}

@article{RN819,
   author = {Tresp, V.},
   title = {A Bayesian committee machine},
   journal = {Neural Comput},
   volume = {12},
   number = {11},
   pages = {2719-41},
   ISSN = {0899-7667 (Print)
0899-7667 (Linking)},
   DOI = {10.1162/089976600300014908},
   url = {https://www.ncbi.nlm.nih.gov/pubmed/11110133},
   year = {2000},
   type = {Journal Article}
}

@article{RN1228,
   author = {Tripathy, Rohit and Bilionis, Ilias and Gonzalez, Marcial},
   title = {Gaussian processes with built-in dimensionality reduction: Applications to high-dimensional uncertainty propagation},
   journal = {Journal of Computational Physics},
   volume = {321},
   pages = {191-223},
   ISSN = {0021-9991},
   year = {2016},
   type = {Journal Article}
}

@article{RN1071,
   author = {Tuo, Rui},
   title = {Adjustments to Computer Models via Projected Kernel Calibration},
   journal = {SIAM/ASA Journal on Uncertainty Quantification},
   volume = {7},
   number = {2},
   pages = {553-578},
   ISSN = {2166-2525},
   DOI = {10.1137/17m1128769},
   url = {<Go to ISI>://WOS:000473215300007},
   year = {2019},
   type = {Journal Article}
}

@article{RN321,
   author = {Ulaganathan, S. and Couckuyt, I. and Dhaene, T. and Degroote, J. and Laermans, E.},
   title = {High dimensional Kriging metamodelling utilising gradient information},
   journal = {Applied Mathematical Modelling},
   volume = {40},
   number = {9-10},
   pages = {5256-5270},
   ISSN = {0307904X},
   DOI = {10.1016/j.apm.2015.12.033},
   url = {<Go to ISI>://WOS:000375511900007},
   year = {2016},
   type = {Journal Article}
}

@article{RN1141,
   author = {van Beek, Anton and Tao, Siyu and Plumlee, Matthew and Apley, Daniel W. and Chen, Wei},
   title = {Integration of Normative Decision-Making and Batch Sampling for Global Metamodeling},
   journal = {Journal of Mechanical Design},
   volume = {142},
   number = {3},
   ISSN = {1050-0472
1528-9001},
   DOI = {10.1115/1.4045601},
   url = {https://doi.org/10.1115/1.4045601},
   year = {2020},
   type = {Journal Article}
}

@inproceedings{RN925,
   author = {Van der Wilk, Mark and Rasmussen, Carl Edward and Hensman, James},
   title = {Convolutional gaussian processes},
   booktitle = {Advances in Neural Information Processing Systems},
   pages = {2849-2858},
   type = {Conference Proceedings}
}

@article{RN1724,
   author = {Villemonteix, Julien and Vazquez, Emmanuel and Walter, Eric},
   title = {An informational approach to the global optimization of expensive-to-evaluate functions},
   journal = {Journal of Global Optimization},
   volume = {44},
   number = {4},
   pages = {509-534},
   ISSN = {1573-2916},
   year = {2009},
   type = {Journal Article}
}

@article{RN1781,
   author = {Villemonteix, Julien and Vazquez, Emmanuel and Walter, Eric},
   title = {An informational approach to the global optimization of expensive-to-evaluate functions},
   journal = {Journal of Global Optimization},
   volume = {44},
   number = {4},
   pages = {509-534},
   ISSN = {1573-2916},
   year = {2009},
   type = {Journal Article}
}

@article{RN298,
   author = {Wang, G. Gary and Shan, S.},
   title = {Review of Metamodeling Techniques in Support of Engineering Design Optimization},
   journal = {Journal of Mechanical Design},
   volume = {129},
   number = {4},
   pages = {370-380},
   ISSN = {1050-0472
1528-9001},
   DOI = {10.1115/1.2429697},
   url = {<Go to ISI>://WOS:000245527800002},
   year = {2007},
   type = {Journal Article}
}

@article{RN1578,
   author = {Wang, Jialei and Clark, Scott C. and Liu, Eric and Frazier, Peter I.},
   title = {Parallel Bayesian Global Optimization of Expensive Functions},
   journal = {Operations Research},
   volume = {68},
   number = {6},
   pages = {1850-1865},
   ISSN = {0030-364X},
   DOI = {10.1287/opre.2019.1966},
   url = {https://doi.org/10.1287/opre.2019.1966},
   year = {2020},
   type = {Journal Article}
}

@article{RN1780,
   author = {Wang, Jialei and Clark, Scott C and Liu, Eric and Frazier, Peter I},
   title = {Parallel Bayesian global optimization of expensive functions},
   journal = {Operations Research},
   volume = {68},
   number = {6},
   pages = {1850-1865},
   ISSN = {0030-364X},
   year = {2020},
   type = {Journal Article}
}

@article{RN1138,
   author = {Wang, Liwei and Chan, Yu-Chin and Liu, Zhao and Zhu, Ping and Chen, Wei},
   title = {Data-driven metamaterial design with Laplace-Beltrami spectrum as “shape-DNA”},
   journal = {Structural and Multidisciplinary Optimization},
   volume = {61},
   number = {6},
   pages = {2613-2628},
   ISSN = {1615-147X
1615-1488},
   DOI = {10.1007/s00158-020-02523-5},
   url = {https://doi.org/10.1007/s00158-020-02523-5},
   year = {2020},
   type = {Journal Article}
}

@article{RN1573,
   author = {Wang, Liwei and Yerramilli, Suraj and Iyer, Akshay and Apley, Daniel and Zhu, Ping and Chen, Wei},
   title = {Scalable Gaussian Processes for Data-Driven Design Using Big Data With Categorical Factors},
   journal = {Journal of Mechanical Design},
   volume = {144},
   number = {2},
   ISSN = {1050-0472},
   DOI = {10.1115/1.4052221},
   url = {https://doi.org/10.1115/1.4052221},
   year = {2021},
   type = {Journal Article}
}

@article{RN276,
   author = {Wang, Xianhui and Shi, Lei},
   title = {A new metamodel method using Gaussian process based bias function for vehicle crashworthiness design},
   journal = {International Journal of Crashworthiness},
   volume = {19},
   number = {3},
   pages = {311-321},
   ISSN = {1358-8265
1754-2111},
   DOI = {10.1080/13588265.2014.898932},
   url = {<Go to ISI>://WOS:000333879700009},
   year = {2014},
   type = {Journal Article}
}

@article{RN1761,
   author = {Wang, Yifan and Chen, Tai-Ying and Vlachos, Dionisios G},
   title = {NEXTorch: a design and Bayesian optimization toolkit for chemical sciences and engineering},
   journal = {Journal of Chemical Information and Modeling},
   volume = {61},
   number = {11},
   pages = {5312-5319},
   ISSN = {1549-9596},
   year = {2021},
   type = {Journal Article}
}

@article{RN1424,
   author = {Wang, Yiqun and Iyer, Akshay and Chen, Wei and Rondinelli, James M.},
   title = {Featureless adaptive optimization accelerates functional electronic materials design},
   journal = {Applied Physics Reviews},
   volume = {7},
   number = {4},
   pages = {041403},
   ISSN = {1931-9401},
   year = {2020},
   type = {Journal Article}
}

@article{RN817,
   author = {Williams, Christopher KI and Rasmussen, Carl Edward and Scwaighofer, A and Tresp, Volker},
   title = {Observations on the Nyström method for Gaussian process prediction},
   year = {2002},
   type = {Journal Article}
}

@inproceedings{RN1256,
   author = {Wilson, Andrew and Adams, Ryan},
   title = {Gaussian process kernels for pattern discovery and extrapolation},
   pages = {1067-1075},
   type = {Conference Proceedings}
}

@article{RN1393,
   author = {Wilson, James T. and Moriconi, Riccardo and Hutter, Frank and Deisenroth, Marc Peter},
   title = {The reparameterization trick for acquisition functions},
   journal = {arXiv preprint arXiv:1712.00424},
   year = {2017},
   type = {Journal Article}
}

@misc{RN1577,
   volume = {115},
   pages = {788--798},
   url = {https://proceedings.mlr.press/v115/wu20a.html},
   year = {2020},
   type = {Conference Paper}
}

@article{RN1425,
   author = {Xu, Hongyi},
   title = {Constructing Oscillating Function-Based Covariance Matrix to Allow Negative Correlations in Gaussian Random Field Models for Uncertainty Quantification},
   journal = {Journal of Mechanical Design},
   volume = {142},
   number = {7},
   ISSN = {1050-0472},
   year = {2020},
   type = {Journal Article}
}

@inproceedings{RN342,
   author = {Zhang, Linmiao and Lei, Yong and Chen, Nan},
   title = {Modeling tunnel profile using Gaussian process},
   booktitle = {Industrial Engineering and Engineering Management (IEEM), 2015 IEEE International Conference on},
   publisher = {IEEE},
   pages = {1352-1356},
   ISBN = {1467380660},
   type = {Conference Proceedings}
}

@article{RN341,
   author = {Zhang, Linmiao and Wang, Kaibo and Chen, Nan},
   title = {Monitoring wafer geometric quality using additive gaussian process model},
   journal = {IIE Transactions},
   year = {2015},
   type = {Journal Article}
}

@article{RN1215,
   author = {Zhang, Qiong and Chien, Peter and Liu, Qing and Xu, Li and Hong, Yili},
   title = {Mixed-input Gaussian process emulators for computer experiments with a large number of categorical levels},
   journal = {Journal of Quality Technology},
   pages = {1-11},
   ISSN = {0022-4065
2575-6230},
   DOI = {10.1080/00224065.2020.1778431},
   url = {https://doi.org/10.1080/00224065.2020.1778431},
   year = {2020},
   type = {Journal Article}
}

@article{RN1375,
   author = {Zhang, Y. and Apley, D. W. and Chen, W.},
   title = {Bayesian Optimization for Materials Design with Mixed Quantitative and Qualitative Variables},
   journal = {Sci Rep},
   volume = {10},
   number = {1},
   pages = {4924},
   ISSN = {2045-2322 (Electronic)
2045-2322 (Linking)},
   DOI = {10.1038/s41598-020-60652-9},
   url = {https://www.ncbi.nlm.nih.gov/pubmed/32188873},
   year = {2020},
   type = {Journal Article}
}

@article{RN693,
   author = {Zhang, Yulei and Notz, William I.},
   title = {Computer Experiments with Qualitative and Quantitative Variables: A Review and Reexamination},
   journal = {Quality Engineering},
   volume = {27},
   number = {1},
   pages = {2-13},
   ISSN = {0898-2112
1532-4222},
   DOI = {10.1080/08982112.2015.968039},
   url = {<Go to ISI>://WOS:000346836700002},
   year = {2014},
   type = {Journal Article}
}

@article{RN1075,
   author = {Zhang, Yichi and Tao, Siyu and Chen, Wei and Apley, Daniel W.},
   title = {A Latent Variable Approach to Gaussian Process Modeling with Qualitative and Quantitative Factors},
   journal = {Technometrics},
   volume = {62},
   number = {3},
   pages = {291-302},
   ISSN = {0040-1706
1537-2723},
   DOI = {10.1080/00401706.2019.1638834},
   url = {<Go to ISI>://WOS:000481877700001},
   year = {2019},
   type = {Journal Article}
}

@article{RN409,
   author = {Zhao, Liang and Choi, K. K. and Lee, Ikjin},
   title = {Metamodeling Method Using Dynamic Kriging for Design Optimization},
   journal = {AIAA Journal},
   volume = {49},
   number = {9},
   pages = {2034-2046},
   ISSN = {0001-1452
1533-385X},
   DOI = {10.2514/1.J051017},
   url = {<Go to ISI>://WOS:000295207100018},
   year = {2011},
   type = {Journal Article}
}

@article{RN1220,
   author = {Zhao, Zhikuan and Fitzsimons, Jack K. and Fitzsimons, Joseph F.},
   title = {Quantum-assisted Gaussian process regression},
   journal = {Physical Review A},
   volume = {99},
   number = {5},
   pages = {052331},
   ISSN = {2469-9926
2469-9934},
   DOI = {10.1103/PhysRevA.99.052331},
   url = {https://link.aps.org/doi/10.1103/PhysRevA.99.052331},
   year = {2019},
   type = {Journal Article}
}

@article{RN545,
   author = {Bessa, M. A. and Bostanabad, R. and Liu, Z. and Hu, A. and Apley, D. W. and Brinson, C. and Chen, W. and Liu, W. K.},
   title = {A framework for data-driven analysis of materials under uncertainty: Countering the curse of dimensionality},
   journal = {Computer Methods in Applied Mechanics and Engineering},
   volume = {320},
   pages = {633-667},
   ISSN = {0045-7825},
   DOI = {10.1016/j.cma.2017.03.037},
   url = {<Go to ISI>://WOS:000402212200025},
   year = {2017},
   type = {Journal Article}
}

@article{RN1163,
   author = {Bostanabad, R.},
   title = {Reconstruction of 3D Microstructures from 2D Images via Transfer Learning},
   journal = {Computer-Aided Design},
   volume = {128},
   pages = {102906},
   ISSN = {0010-4485},
   DOI = {ARTN 102906
10.1016/j.cad.2020.102906},
   url = {<Go to ISI>://WOS:000567397500006},
   year = {2020},
   type = {Journal Article}
}

@article{RN6,
   author = {Bostanabad, Ramin and Bui, Anh Tuan and Xie, Wei and Apley, Daniel W and Chen, Wei},
   title = {Stochastic microstructure characterization and reconstruction via supervised learning},
   journal = {Acta Materialia},
   volume = {103},
   pages = {89-102},
   ISSN = {1359-6454},
   year = {2016},
   type = {Journal Article}
}

@article{RN940,
   author = {Bostanabad, R. and Chan, Y. C. and Wang, L. W. and Zhu, P. and Chen, W.},
   title = {Globally Approximate Gaussian Processes for Big Data With Application to Data-Driven Metamaterials Design},
   journal = {Journal of Mechanical Design},
   volume = {141},
   number = {11},
   ISSN = {1050-0472},
   DOI = {Artn 111402
10.1115/1.4044257},
   url = {<Go to ISI>://WOS:000506891900010},
   year = {2019},
   type = {Journal Article}
}

@article{RN184,
   author = {Bostanabad, R. and Chen, W. and Apley, D. W.},
   title = {Characterization and reconstruction of 3D stochastic microstructures via supervised learning},
   journal = {J Microsc},
   volume = {264},
   number = {3},
   pages = {282-297},
   ISSN = {1365-2818 (Electronic)
0022-2720 (Linking)},
   DOI = {10.1111/jmi.12441},
   url = {https://www.ncbi.nlm.nih.gov/pubmed/27378619},
   year = {2016},
   type = {Journal Article}
}

@article{RN783,
   author = {Bostanabad, R. and Kearney, T. and Tao, S. Y. and Apley, D. W. and Chen, W.},
   title = {Leveraging the nugget parameter for efficient Gaussian process modeling},
   journal = {International Journal for Numerical Methods in Engineering},
   volume = {114},
   number = {5},
   pages = {501-516},
   ISSN = {0029-5981},
   DOI = {10.1002/nme.5751},
   url = {<Go to ISI>://WOS:000428998100002},
   year = {2018},
   type = {Journal Article}
}

@inbook{RN899,
   author = {Bostanabad, Ramin and Liang, Biao and Gao, Jiaying and Liu, Wing Kam and Cao, Jian and Zeng, Danielle and Su, Xuming and Xu, Hongyi and Li, Yang and Chen, Wei},
   title = {Multiscale Simulation of Fiber Composites with Spatially-Varying Uncertainties},
   booktitle = {Uncertainty Quantification in Multiscale Materials Modeling},
   publisher = {Elsevier},
   year = {2019},
   type = {Book Section}
}

@article{RN704,
   author = {Bostanabad, R. and Liang, B. and Gao, J. Y. and Liu, W. K. and Cao, J. and Zeng, D. and Su, X. M. and Xu, H. Y. and Li, Y. and Chen, W.},
   title = {Uncertainty quantification in multiscale simulation of woven fiber composites},
   journal = {Computer Methods in Applied Mechanics and Engineering},
   volume = {338},
   pages = {506-532},
   ISSN = {0045-7825},
   DOI = {10.1016/j.cma.2018.04.024},
   url = {<Go to ISI>://WOS:000436490700021},
   year = {2018},
   type = {Journal Article}
}

@article{RN680,
   author = {Bostanabad, R. and Zhang, Y. C. and Li, X. L. and Kearney, T. and Brinson, L. C. and Apley, D. W. and Liu, W. K. and Chen, W.},
   title = {Computational microstructure characterization and reconstruction: Review of the state-of-the-art techniques},
   journal = {Progress in Materials Science},
   volume = {95},
   pages = {1-41},
   ISSN = {0079-6425},
   DOI = {10.1016/j.pmatsci.2018.01.005},
   url = {<Go to ISI>://WOS:000431163100001},
   year = {2018},
   type = {Journal Article}
}

@article{RN1654,
   author = {Chen, W. and Iyer, A. and Bostanabad, R.},
   title = {Data Centric Design: A New Approach to Design of Microstructural Material Systems},
   journal = {Engineering},
   volume = {10},
   pages = {89-98},
   ISSN = {2095-8099},
   DOI = {10.1016/j.eng.2021.05.022},
   url = {<Go to ISI>://WOS:000807736400013},
   year = {2022},
   type = {Journal Article}
}

@article{RN1656,
   author = {Deng, Shiguang and Apelian, Diran and Bostanabad, Ramin},
   title = {Concurrent Multiscale Damage Analysis with Adaptive Spatiotemporal Dimension Reduction},
   journal = {arXiv preprint arXiv:2205.12149},
   year = {2022},
   type = {Journal Article}
}

@article{RN1786,
   author = {Deng, Shiguang and Mora, Carlos and Apelian, Diran and Bostanabad, Ramin},
   title = {Data-Driven Calibration of Multi-Fidelity Multiscale Fracture Models via Latent Map Gaussian Process},
   journal = {Journal of Mechanical Design},
   pages = {1-15},
   ISSN = {1050-0472},
   DOI = {10.1115/1.4055951},
   url = {https://doi.org/10.1115/1.4055951},
   year = {2022},
   type = {Journal Article}
}

@misc{RN1692,
   year = {2022},
   type = {Conference Paper}
}

@article{RN1655,
   author = {Deng, S. G. and Soderhjelm, C. and Apelian, D. and Bostanabad, R.},
   title = {Reduced-order multiscale modeling of plastic deformations in 3D alloys with spatially varying porosity by deflated clustering analysis},
   journal = {Computational Mechanics},
   pages = {1-32},
   ISSN = {0178-7675},
   DOI = {10.1007/s00466-022-02177-8},
   url = {<Go to ISI>://WOS:000809539000003},
   year = {2022},
   type = {Journal Article}
}

@article{RN1633,
   author = {Eweis-Labolle, Jonathan Tammer and Oune, Nicholas and Bostanabad, Ramin},
   title = {Data Fusion With Latent Map Gaussian Processes},
   journal = {Journal of Mechanical Design},
   volume = {144},
   number = {9},
   pages = {1-41},
   ISSN = {1050-0472},
   DOI = {10.1115/1.4054520},
   url = {https://doi.org/10.1115/1.4054520},
   year = {2022},
   type = {Journal Article}
}

@article{RN681,
   author = {Hassaninia, I. and Bostanabad, R. and Chen, W. and Mohseni, H.},
   title = {Characterization of the Optical Properties of Turbid Media by Supervised Learning of Scattering Patterns},
   journal = {Sci Rep},
   volume = {7},
   number = {1},
   pages = {15259},
   ISSN = {2045-2322 (Electronic)
2045-2322 (Linking)},
   DOI = {10.1038/s41598-017-15601-4},
   url = {https://www.ncbi.nlm.nih.gov/pubmed/29127385},
   year = {2017},
   type = {Journal Article}
}

@article{RN1024,
   author = {Mozaffar, M. and Bostanabad, R. and Chen, W. and Ehmann, K. and Cao, J. and Bessa, M. A.},
   title = {Deep learning predicts path-dependent plasticity},
   journal = {Proc Natl Acad Sci U S A},
   volume = {116},
   number = {52},
   pages = {26414-26420},
   ISSN = {1091-6490 (Electronic)
0027-8424 (Linking)},
   DOI = {10.1073/pnas.1911815116},
   url = {https://www.ncbi.nlm.nih.gov/pubmed/31843918},
   year = {2019},
   type = {Journal Article}
}

@article{RN1559,
   author = {Oune, N. and Bostanabad, R.},
   title = {Latent map Gaussian processes for mixed variable metamodeling},
   journal = {Computer Methods in Applied Mechanics and Engineering},
   volume = {387},
   pages = {114128},
   ISSN = {0045-7825},
   DOI = {ARTN 114128
10.1016/j.cma.2021.114128},
   url = {<Go to ISI>://WOS:000708647400003},
   year = {2021},
   type = {Journal Article}
}

@misc{RN1383,
   volume = {84003},
   pages = {V11AT11A004},
   month = {2020},
   ISBN = {0791884007},
   year = {2020},
   type = {Conference Paper}
}

@article{RN1558,
   author = {Planas, R. and Oune, N. and Bostanabad, R.},
   title = {Evolutionary Gaussian Processes},
   journal = {Journal of Mechanical Design},
   volume = {143},
   number = {11},
   pages = {111703},
   ISSN = {1050-0472},
   DOI = {Artn 111703
10.1115/1.4050746},
   url = {<Go to ISI>://WOS:000702466200013},
   year = {2021},
   type = {Journal Article}
}

@article{RN1384,
   author = {Suh, Y. and Bostanabad, R. and Won, Y.},
   title = {Deep learning predicts boiling heat transfer},
   journal = {Sci Rep},
   volume = {11},
   number = {1},
   pages = {5622},
   ISSN = {2045-2322 (Electronic)
2045-2322 (Linking)},
   DOI = {10.1038/s41598-021-85150-4},
   url = {https://www.ncbi.nlm.nih.gov/pubmed/33692489},
   year = {2021},
   type = {Journal Article}
}

@inproceedings{RN649,
   author = {Tao, Siyu and Shintani, Kohei and Bostanabad, Ramin and Chan, Yu-Chin and Yang, Guang and Meingast, Herb and Chen, Wei},
   title = {Enhanced Gaussian Process Metamodeling and Collaborative Optimization for Vehicle Suspension Design Optimization},
   booktitle = {ASME 2017 International Design Engineering Technical Conferences and Computers and Information in Engineering Conference},
   publisher = {American Society of Mechanical Engineers},
   volume = {2B},
   type = {Conference Proceedings}
}

@article{RN1637,
   author = {Wang, Hengjie and Planas, Robert and Chandramowlishwaran, Aparna and Bostanabad, Ramin},
   title = {Mosaic flows: A transferable deep learning framework for solving PDEs on unseen domains},
   journal = {Computer Methods in Applied Mechanics and Engineering},
   volume = {389},
   pages = {114424},
   ISSN = {00457825},
   DOI = {10.1016/j.cma.2021.114424},
   url = {https://www.sciencedirect.com/science/article/pii/S004578252100668X},
   year = {2022},
   type = {Journal Article}
}

@article{RN791,
   author = {Zhang, W. Z. and Bostanabad, R. and Liang, B. and Su, X. M. and Zeng, D. and Bessa, M. A. and Wang, Y. C. and Chen, W. and Cao, J.},
   title = {A numerical Bayesian-calibrated characterization method for multiscale prepreg preforming simulations with tension-shear coupling},
   journal = {Composites Science and Technology},
   volume = {170},
   pages = {15-24},
   ISSN = {0266-3538},
   DOI = {10.1016/j.compscitech.2018.11.019},
   url = {<Go to ISI>://WOS:000456228100003},
   year = {2019},
   type = {Journal Article}
}

@phdthesis{RN1788,
   author = {Bostanabad, Ramin},
   title = {Quantification of Microstructure Induced Uncertainty in Multiscale Materials with Random Processes},
   university = {Northwestern University},
   year = {2019},
   type = {Thesis}
}

@inproceedings{RN1789,
   author = {Takeno, Shion and Fukuoka, Hitoshi and Tsukada, Yuhki and Koyama, Toshiyuki and Shiga, Motoki and Takeuchi, Ichiro and Karasuyama, Masayuki},
   title = {Multi-fidelity Bayesian optimization with max-value entropy search and its parallelization},
   booktitle = {International Conference on Machine Learning},
   publisher = {PMLR},
   pages = {9334-9345},
   ISBN = {2640-3498},
   type = {Conference Proceedings}
}

@article{RN1790,
   author = {Renganathan, S Ashwin and Rao, Vishwas and Navon, Ionel M},
   title = {CAMERA: A Method for Cost-aware, Adaptive, Multifidelity, Efficient Reliability Analysis},
   journal = {arXiv preprint arXiv:2203.01436},
   year = {2022},
   type = {Journal Article}
}

@article{RN1794,
   author = {Tran, Anh and Tranchida, Julien and Wildey, Tim and Thompson, Aidan P.},
   title = {Multi-fidelity machine-learning with uncertainty quantification and Bayesian optimization for materials design: Application to ternary random alloys},
   journal = {The Journal of Chemical Physics},
   volume = {153},
   number = {7},
   pages = {074705},
   DOI = {10.1063/5.0015672},
   url = {https://aip.scitation.org/doi/abs/10.1063/5.0015672},
   year = {2020},
   type = {Journal Article}
}


==> 16_OLD.tex <==
\cmt{The common scenario in MFBO problems is that there are different data sources whose accuracy level is different;  the objective is to emulate the HF which faces the following constraints: (1) mixed input data; (2) limited data from HF; and (3) lack of knowledge about how diverse data sources are related to one another. 
As noted in section~\ref{sec: background-LMGP}, LMGP is the extension of GPs that incorporates a newly developed correlation function that enables LMGP to handle categorical data as well. Therefore, the first restriction is satisfied by utilizing LMGP as a surrogate model.

A recent study demonstrates that LMGP is a potent tool in data fusion field \cite{oune2021data}, which helps us to satisfy the second constraint—namely limited data from HF. In this study, it is demonstrated through numerous examples with various dimensionalities that the LMGP is able to approximate the HF surrogate by fusing the limited HF data with more  LF data. In order to execute data fusion using LMGP, we should add a column to the inputs to distinguish among different fidelity sources. For example, if there are 4 different data sources, a categorical feature t={0,1,2,3} will be appended to the input. Each level of this categorical feature corresponds to a certain data source (for instance, $0$ represents the HF, $1$ represents the first LF, etc.) and will be appended to the sample that originates from that source of data:
%=================================================
\begin{equation} 
    \begin{split}
        \boldsymbol{X}=\left[\begin{array}{cc}
        \boldsymbol{X}_h & \mathbf{0}_{n_h \times 1} \\
        \boldsymbol{X}_{l_1} & 1 \times \mathbf{1}_{n_{l_1 \times 1}} \\
        \boldsymbol{X}_{l_2} & 2 \times \mathbf{1}_{n_{l_1 \times 1}} \\
        \boldsymbol{X}_{l_3} & 3 \times \mathbf{1}_{n_{l_1} \times 1}
        \end{array}\right] \text { and } \boldsymbol{Y}=\left[\begin{array}{c}
        \boldsymbol{y}_h \\
        \boldsymbol{y}_{l_1} \\
        \boldsymbol{y}_{l_2} \\
        \boldsymbol{y}_{l_3}
        \end{array}\right]  \label{LMGP-fidelity-append}
    \end{split}
\end{equation}
%=================================================

\unindent Where $ \mathbf{1}_{n \times 1}$ is an $ n \times 1$ vector of ones. Then, this combined data will be fed into LMGP model. Combining the expensive limited HF data with more LF data, we have enough initial data on which train our model and approximate the HF. 
 In order to use the majority of existing MF methods, the hierarchy of the fidelities and their correlation must be determined\cite{winter2022stochastic}; for example, some methods are only eligible for linear correlation \cite{sobester2008engineering}, \cite{perdikaris2016model}, \cite{perdikaris2016multifidelity}, some for non-linear correlation\cite{perdikaris2017nonlinear}, etc. However, LMGP does not need to know the correlation among fidelities or even their hierarchy—which is the underlaying assumption of LMGP; this assumption is the key factor that makes LMGP superior to its data fusion counterparts.
As mentioned in section~\ref{sec:LMGP}, there are two sets of hyperparameters that should be estimated in LMGP, e.g., $\boldsymbol{\hat{\omega}}$ and $\boldsymbol{\hat{A}}$ which are shared among numerical and categorical inputs, respectively. As the hyperparameters are shared among all the data, they construct the connection among the data sources. Hence, regardless of how the correlation of fidelities is, estimating the hyperparameters results in the estimation of both the distribution and correlation of all the data sources.

The last constraint is crucial since MF approaches are most practical for the cases where fidelities are correlated; if fidelities are not correlated, LF sources could act as noise to the HF source and exacerbate the convergence process, so MF fails to work. Therefore, having a criterion in mind to distinguish the suitability of the LF source to HF based on their correlation-level is essential ; 
We use the latent map feature in the LMGP model to decide on the suitability of the LF sources. The learned latent space is based on the correlation among the distribution of fidelity sources. In this regard, the closer two points are in the latent space, the more correlated they are. The latent maps are able to display the correlation of the fidelities by applying MLE method.The goal of MLE is to estimate the hyperparameters for which the observed data have the highest joint probability. Denoting hyperparameters by $\boldsymbol{\theta}=\left[\theta_1, \theta_2, \ldots, \theta_k\right]^{\top}$ and observed data samples by $\mathbf{y}=\left(y_1, y_2, \ldots, y_n\right)$ the likelihood of MLE is defined as:
%=================================================
\begin{equation} 
        \begin{split}     \mathcal{L}_n(\boldsymbol{\theta})=\mathcal{L}_n(\boldsymbol{\theta} ; \mathbf{y})=f_n(\mathbf{y} ; \boldsymbol{\theta})    
        \end{split}
    \label{eq:MLE}
\end{equation}
%=================================================
\noindent after constructing the likelihood, MLE estimates the hyperparameters by finding the distribution from which the data most likely come (maximizing the likelihood function over the parameter space):
%=================================================
\begin{equation} 
        \begin{split}     \hat{\boldsymbol{\theta}}=\underset{\boldsymbol{\theta} \in \Theta}{\arg \max } \mathcal{L}_n(\boldsymbol{\theta} ; \mathbf{y})   
        \end{split}
    \label{eq:MLE-point-estimate}
\end{equation}
%=================================================

As an illustration, consider the Borehole example with five different fidelity sources which will be explained in detail in section~\ref{sec: Results}. Figure~\ref{fig:Borehole-fidelity} shows the latent map of the LMGP model trained on the Borehole's initial data. Based on this figure, the HF is highly correlated with the fourth and fifth LFs, while the first two LFs are not correlated to the HF, and using them does not aid for the convergence process.   
%=================================================================================
\begin{figure*}[!b] 
	\centering
	\includegraphics[page=1, width = 0.8\textwidth]{figures/borehole_fidelity.pdf}
	\vspace{-0.3cm}
	\caption{\textbf{Latent map of Borehole example:} Each point denotes a source of data and the distance among them is an indication of their correlation. With this regard, the first two LF sources are not correlated with the HF source and using them in the optimization exacerbates the convergence.}
   \label{fig:Borehole-fidelity}
\end{figure*}
}
%=================================================================================

Guiding optimization to find the most efficient samples by balancing exploration and exploitation, makes AFs to be a crucial ingredient of BO in SF problems. However, defining AF for MF problems is more challenging, since in MF problems, the AF trades off between information gain and cost, as well as exploration and exploitation to find the most efficient sample and its corresponding fidelity.

In a typical SF black-box optimization problem, the more samples we take, the more certain search space we will have which paves the convenient way for finding the optimum. However, the drawback of this approach is the total expense, since we usually aim to optimize the HF function which is expensive and merely sampling from it could exhaust the budget before finding the optimum point. As explained in Sec.\ref{sec: existing_MFBO}, this drawback is resolved in MF problems as the main premise in MF problems is to take many inexpensive LF samples all over the domain (high exploration) to reduce the uncertainty of the whole space; then, AF finds the next point by exploiting the more certain HF domain through fewer samples. So, we aim to propose an AF, the goal of which is to do more exploration in LF domain and more exploitation in HF’s. Due to the difference in the sampling criteria in high and low fidelity domains, we define two distinct AFs designed for the criteria of each space. 

Regarding the aforementioned, we want to define a utility function for LF domain which samples the points that improve $y^*$ by favoring exploration. Based on Sec.\ref{sec: AFs}, in a maximization problem improvement can be defined as $y(\boldsymbol{x})–y^*$. Utilizing reparameterization trick by defining $z\sim \mathcal{N}(0,1)$ with standard normal distribution ($\phi(z)=\frac{1}{\sqrt{2 \pi}} \exp \left(-z^2 / 2\right)$), the improvement can be rewritten as:
%=================================================
\begin{equation} 
    \begin{split}
        y(\boldsymbol{x}) - y^*= \mu(\boldsymbol{x})+ \sigma(\boldsymbol{x})z- y^*
    \end{split}
    \label{eq: LF-rewrite-u}
\end{equation}
%=================================================
\noindent In the above formulation, $\sigma(\boldsymbol{x})z$ is the part in charge of exploration, since it directly deals with uncertainty $\sigma(\boldsymbol{x})$. Therefore, we can ignore other terms and propose the utility function for LF domain with focus on exploration as:
%=================================================
\begin{equation} 
    \begin{split}
        I_{LF}(\boldsymbol{x})= \begin{cases}\sigma(\boldsymbol{x})z& y(\boldsymbol{x})>y^* \\ 0 & y(\boldsymbol{x}) \leq y^*\end{cases}
    \end{split}
    \label{eq: LF-utility}
\end{equation}
%=================================================
\noindent now, the corresponding AF can be calculated by substituting the proposed utility function in Eq.\ref{eq: general-AF}:
%=================================================
\begin{equation} 
    \begin{split}
        \alpha_{LF}(\boldsymbol{x})=\int_{-\infty}^{\infty} I_{LF}(\boldsymbol{x}) \phi(z) \mathrm{d} z=\int_{-\infty}^{\infty} \sigma(\boldsymbol{x})z \phi(z) \mathrm{d} z
    \end{split}
    \label{eq: LF-CA-AF}
\end{equation}
%=================================================
\noindent the integral is zero for $y(\boldsymbol{x}) < y^*$, so finding the switch point simplifies the calculation of the integral: 
%=================================================
\begin{equation} 
    \begin{split}
        y(\boldsymbol{x})=y^* \Rightarrow \mu(\boldsymbol{x})+\sigma(\boldsymbol{x}) z=y^* \Rightarrow z_{0}=\frac{y^*-\mu(\boldsymbol{x})}{\sigma(\boldsymbol{x})}
    \end{split}
    \label{eq:LF_AF_switch}
\end{equation}
%=================================================
\noindent now we can calculate the integral:
%=================================================
\begin{equation} 
    \begin{split}
        \begin{aligned}
        &\alpha_{L F}(\boldsymbol{x})=\int_{z_0}^{\infty} \sigma(\boldsymbol{x}) z \phi(z) d(z)\\
        &=\int_{z_0}^{\infty} \frac{\sigma(\boldsymbol{x}) z}{\sqrt{2 \pi}} e^{-\frac{z^2}{2}} d(z)\\
        &=\frac{\sigma(\boldsymbol{x})}{\sqrt{2 \pi}} \int_{z_0}^{\infty} z e^{-\frac{z^2}{2}} d(z)=-\frac{\sigma(\boldsymbol{x})}{\sqrt{2 \pi}} \int_{z_0}^{\infty}(e^{-\frac{z^2}{2}})^{\prime} d(z)\\
        &=-\frac{\sigma(\boldsymbol{x})}{\sqrt{2 \pi}}[e^{-\frac{z^2}{2}}]_{z_0}^{\infty}\\
        &=\sigma(\boldsymbol{x}) \phi(z_0) \\
        &= \sigma(\boldsymbol{x}) \phi(\frac{y^* - \mu(\boldsymbol{x})}{\sigma(\boldsymbol{x})})
        \end{aligned}
    \end{split}
    \label{eq:LF_AF}
\end{equation}
%=================================================
\noindent where $\phi$ is a PDF of a standard normal distribution, $\mu(\boldsymbol{x})$ and $\sigma(\boldsymbol{x})$ are defined in Eq.\ref{eq: LMGP-predict} and Eq.\ref{eq: LMGP-posterio-cov}. Comparing our proposed AF with Eq.\ref{eq:EI-AF-compl}, one finds out that it is the same as the exploration part of EI.

PI is the AF we deployed for the HF domain, due to ts explicit form, low computational cost, excellent performance and focus on exploitation:
%=================================================
\begin{equation} 
    \begin{split}
        \alpha_{HF}(\boldsymbol{x})=\Phi(\frac{\mu(\boldsymbol{x})-y^*}{\sigma(\boldsymbol{x})})
    \end{split}
    \label{eq: HF-AF}
\end{equation}
%=================================================
\noindent where $\Phi$ denotes the CDF of a standard normal distribution. In each iteration, low and high fidelity data will be fed into their corresponding AFs, the AFs calculate the acquisition value of each point; finally, the next sample and its fidelity source are achievable through an auxiliary optimization problem. 

In normal distributions, PDF is greater than CDF for points less than the mean, however, by passing the mean, CDF increases dramatically while PDF decreases. In a maximization problem, we aim to find a point which improves \fbest ~($\mu(\boldsymbol{x}) > y^*$), therefore $\frac{\mu(\boldsymbol{x})-y^*}{\sigma(\boldsymbol{x})}$ is a positive value (larger than mean) which causes the acquisition value of HF be larger than LF's; consequently, the AF mostly samples from the expensive HF source instead of low-cost LF source. To address this discrepancy, we divide the AFs by the cost of their corresponding fidelity source to make them cost-aware and balance between information gain and cost. Then, assuming we aim to maximize source $l \in \{1,...,ds\}$, the proposed novel cost-aware AFs for LF and HF data are, respectively:
%=================================================
\begin{equation} 
    \begin{split}
       \alpha_{LF}(\boldsymbol{x}_{s_{(j \neq{l})}})=\frac{\sigma(\boldsymbol{x}_{s_{(j \neq{l})}}) \phi(\frac{y^*-\mu(\boldsymbol{x}_{s_{(j \neq{l})}})}{\sigma(\boldsymbol{x}_{s_{(j \neq{l})}})})}{C_{s_{(j \neq{l})}}}
    \end{split}
    \label{eq:LF_CA_AF}
\end{equation}
%=================================================
%=================================================
\begin{equation} 
    \begin{split}
       \alpha_{HF}(\boldsymbol{x}_{s_{(l)}})=\frac{\Phi(\frac{\mu(\boldsymbol{x}_{s_{(l)}})-y^*}{\sigma(\boldsymbol{x}_{s_{(l)}})})}{C_{s_{(l)}}}
    \end{split}
    \label{eq:HF_CA_AF}
\end{equation}
%=================================================
\noindent where $\boldsymbol{x}_{s_{(j)}}$ and $C_{s_{(j)}}$ denote the data and its corresponding cost from $j^{th}$ data source, respectively. Finally, we propose an auxiliary optimization problem to find the next sample ($k^{th}$ sample) and its fidelity source ($s$):
%=================================================
\begin{equation} 
    \begin{split}
       \boldsymbol{x}_{s}^k=\operatorname{argmax}[\alpha_{HF}(\boldsymbol{x}_{s_{(l)}}), \alpha_{LF}(\boldsymbol{x}_{s_{(j \neq{l})}})]
    \end{split}
    \label{eq:auxiliary}
\end{equation}
%=================================================
\noindent where $\boldsymbol{x}_{(s)}^k$ denotes the sample taken in iteration $k$ from data source $s$ and $\boldsymbol{x}_{s_{(j \neq{l})}})$ indicates all the fidelity sources except the source we want to maximize $(l)$. Now, because the LF data is much cheaper than HF data, the algorithm will mostly sample from LF and only takes a few samples from HF, which provides it with a very large amount of information to compensate the cost difference.

A crucial point to consider in MFBO problems is guaranteeing the convergence to the optimum of the HF source (ground truth) not LF's. For instance, in a minimization problem in which the minimum of LF is lower than that of HF's; how we can force the AF to distinguish between HF and LF and find the ground truth? \fbest is an approximation of the ground truth in our proposed utility functions. Every time that the AF query a point with lower objective value, \fbest will be updated and it remains fixed whenever there be no improvement in the objective value. Therefore, by constraining \fbest to be merely updated by the improvement in HF samples, we guarantee the convergence of our proposed method to the ground truth.

As an illustration, consider Fig.\ref{fig:1d-curvature} which is a 1-dimensional bi-fidelity example whose LF minimum is lower than HF's. Details and formulation regarding the example are provided in Table.\ref{table: Analytical formulation}. Extreme cost difference between fidelity sources (1000 for HF and 1 for LF) is defined to make the convergence more challenging, since in this situation the AF of HF will be divided by a large number and its value will be smaller than LF's unless the AF finds a point with large enough information to compensate for the extreme cost difference. Fig.\ref{fig:1d-convergence} demonstrates that our proposed MFCA method could find the ground truth while the minimum of LF ($-7.13$) was much lower than that of HF's ($-5.73$) and the LF source was extremely cheaper than HF.   


%======================================

\begin{figure}
\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/1d_cureve_dashed.pdf}
  \caption{}
  \label{fig:1d-curvature}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{figures/1d_convergence_blue_ca.pdf}
  \caption{}
  \label{fig:1d-convergence}
\end{subfigure}
\caption{\textbf{Double-well potential:} $(\boldsymbol{a})$ \textbf{Bias of LF source:} The minimum of LF (blue curve), is lower than HF's to challenge the proposed MFCA method in finding the ground truth while the minimum of LF is lower, however, $(\boldsymbol{b})$ \textbf{Convergence plot:} despite the presence of LF data with a lower minimum, the proposed MFCA method could successfully find the ground truth}
\label{fig:1D-approach}
\end{figure}

\cmt{
%===========================================
\begin{table}[t]
    \caption{\textbf{Relative accuracy of functions for analytical problem}}
    \centering
    \begin{tabular}{ccccc}
        \hline
        \multirow{2}{*}{\textbf{Example}} & \multicolumn{4}{c}{\textbf{RRMSE}} \\ \cline{2-5} 
                                          & LF1     & LF2    & LF3    & LF4    \\ \hline
        Double well potential             & 1.14    & -      & -      & -      \\ \hline
        Rosenbrock                        & 1.42    & -      & -      & -      \\ \hline
        Borehole                          & 4.40    & 1.54   & 1.30   & 1.30   \\ \hline
        Wing                              & 0.19    & 1.14   & 5.75   & -      \\ \hline
        \label{table: RRMSE}
    \end{tabular}
\end{table}
%==========================================
}

\cmt{
\section{MSE of Different MF Emulatrs} \label{appendix_table__mse}

\begin{table}[t]
    \caption{\textbf{MSE of the existing emulators on source 1}}
    \setlength{\extrarowheight}{2pt}
    \setlength{\tabcolsep}{2.5pt}
    {\renewcommand{\arraystretch}{2}}
    \centering
    \begin{tabular}{|c|cccccccccc|}
        \hline
        Sorce 1 & \multicolumn{10}{c|}{Iteration} \\ \hline
        Method &
          \multicolumn{1}{c|}{1} &
          \multicolumn{1}{c|}{2} &
          \multicolumn{1}{c|}{3} &
          \multicolumn{1}{c|}{4} &
          \multicolumn{1}{c|}{5} &
          \multicolumn{1}{c|}{6} &
          \multicolumn{1}{c|}{7} &
          \multicolumn{1}{c|}{8} &
          \multicolumn{1}{c|}{9} &
          10 \\ \hline
        LMGP &
          \multicolumn{1}{c|}{51.2} &
          \multicolumn{1}{c|}{37.82} &
          \multicolumn{1}{c|}{61.63} &
          \multicolumn{1}{c|}{42.51} &
          \multicolumn{1}{c|}{62.55} &
          \multicolumn{1}{c|}{47.4} &
          \multicolumn{1}{c|}{45.1} &
          \multicolumn{1}{c|}{38.77} &
          \multicolumn{1}{c|}{65.96} &
          45.27 \\
        Single-task MF GP &
          \multicolumn{1}{c|}{357.17} &
          \multicolumn{1}{c|}{231.8} &
          \multicolumn{1}{c|}{359.89} &
          \multicolumn{1}{c|}{252.44} &
          \multicolumn{1}{c|}{288.14} &
          \multicolumn{1}{c|}{281} &
          \multicolumn{1}{c|}{185.13} &
          \multicolumn{1}{c|}{250.01} &
          \multicolumn{1}{c|}{302.07} &
          262.72 \\
        Co-kriging &
          \multicolumn{1}{c|}{19.04} &
          \multicolumn{1}{c|}{16.03} &
          \multicolumn{1}{c|}{20.8} &
          \multicolumn{1}{c|}{27.92} &
          \multicolumn{1}{c|}{20.08} &
          \multicolumn{1}{c|}{26.53} &
          \multicolumn{1}{c|}{30.73} &
          \multicolumn{1}{c|}{16.96} &
          \multicolumn{1}{c|}{17.29} &
          40.62 \\ \hline
    \end{tabular}
\end{table}

%==============================================================
\begin{table}[t]
    \caption{\textbf{MSE of the existing emulators on source 2}}
    \setlength{\extrarowheight}{2pt}
    \setlength{\tabcolsep}{2.5pt}
    {\renewcommand{\arraystretch}{2}}
    \centering
    \begin{tabular}{|c|cccccccccc|}
        \hline
        Sorce 2 & \multicolumn{10}{c|}{Iteration} \\ \hline
        Method &
          \multicolumn{1}{c|}{1} &
          \multicolumn{1}{c|}{2} &
          \multicolumn{1}{c|}{3} &
          \multicolumn{1}{c|}{4} &
          \multicolumn{1}{c|}{5} &
          \multicolumn{1}{c|}{6} &
          \multicolumn{1}{c|}{7} &
          \multicolumn{1}{c|}{8} &
          \multicolumn{1}{c|}{9} &
          10 \\ \hline
        LMGP &
          \multicolumn{1}{c|}{2.41} &
          \multicolumn{1}{c|}{8.29} &
          \multicolumn{1}{c|}{1.71} &
          \multicolumn{1}{c|}{1.49} &
          \multicolumn{1}{c|}{3.18} &
          \multicolumn{1}{c|}{2.92} &
          \multicolumn{1}{c|}{1.64} &
          \multicolumn{1}{c|}{2.66} &
          \multicolumn{1}{c|}{4.74} &
          3.98 \\
        Single-task MF GP &
          \multicolumn{1}{c|}{55.08} &
          \multicolumn{1}{c|}{45.65} &
          \multicolumn{1}{c|}{50.25} &
          \multicolumn{1}{c|}{33.02} &
          \multicolumn{1}{c|}{74.42} &
          \multicolumn{1}{c|}{72.54} &
          \multicolumn{1}{c|}{39.71} &
          \multicolumn{1}{c|}{58.60} &
          \multicolumn{1}{c|}{84.21} &
          99.12 \\
        Co-kriging &
          \multicolumn{1}{c|}{1160.09} &
          \multicolumn{1}{c|}{1291.45} &
          \multicolumn{1}{c|}{1136.35} &
          \multicolumn{1}{c|}{1524.26} &
          \multicolumn{1}{c|}{1025.90} &
          \multicolumn{1}{c|}{1344.32} &
          \multicolumn{1}{c|}{1088.24} &
          \multicolumn{1}{c|}{1457.53} &
          \multicolumn{1}{c|}{1477.31} &
          1176.68 \\ \hline
    \end{tabular}
\end{table}

%================================

\begin{table}[t]
    \caption{\textbf{MSE of the existing emulators on source 3}}
    \setlength{\extrarowheight}{2pt}
    \setlength{\tabcolsep}{2.5pt}
    {\renewcommand{\arraystretch}{2}}
    \centering
    \begin{tabular}{|c|cccccccccc|}
        \hline
        Sorce 3 & \multicolumn{10}{c|}{Iteration} \\ \hline
        Method &
          \multicolumn{1}{c|}{1} &
          \multicolumn{1}{c|}{2} &
          \multicolumn{1}{c|}{3} &
          \multicolumn{1}{c|}{4} &
          \multicolumn{1}{c|}{5} &
          \multicolumn{1}{c|}{6} &
          \multicolumn{1}{c|}{7} &
          \multicolumn{1}{c|}{8} &
          \multicolumn{1}{c|}{9} &
          10 \\ \hline
        LMGP &
          \multicolumn{1}{c|}{0.94} &
          \multicolumn{1}{c|}{2.81} &
          \multicolumn{1}{c|}{2.23} &
          \multicolumn{1}{c|}{1.19} &
          \multicolumn{1}{c|}{2.12} &
          \multicolumn{1}{c|}{1.06} &
          \multicolumn{1}{c|}{2.97} &
          \multicolumn{1}{c|}{1.93} &
          \multicolumn{1}{c|}{1.15} &
          2.91 \\
        Single-task MF GP &
          \multicolumn{1}{c|}{34.09} &
          \multicolumn{1}{c|}{54.20} &
          \multicolumn{1}{c|}{96.03} &
          \multicolumn{1}{c|}{18.55} &
          \multicolumn{1}{c|}{54.82} &
          \multicolumn{1}{c|}{37.81} &
          \multicolumn{1}{c|}{32.24} &
          \multicolumn{1}{c|}{39.68} &
          \multicolumn{1}{c|}{24.87} &
          72.74 \\
        Co-kriging &
          \multicolumn{1}{c|}{1084.67} &
          \multicolumn{1}{c|}{1165.69} &
          \multicolumn{1}{c|}{1248.97} &
          \multicolumn{1}{c|}{1150.65} &
          \multicolumn{1}{c|}{1082.05} &
          \multicolumn{1}{c|}{1133.42} &
          \multicolumn{1}{c|}{968.82} &
          \multicolumn{1}{c|}{831.86} &
          \multicolumn{1}{c|}{1011.70} &
          1075.15 \\ \hline
    \end{tabular}
\end{table}
%====================
}

In this Section, to assess the performance of $LMGP_{CA}$ we deploy two real-world datasets: the Material design dataset \cite{oune2021latent} and  Hybrid Organic–Inorganic Perovskite (HOIP) dataset \cite{herbol2020cost}. Since both examples involve categorical features that $BoTorch$ cannot handle, we only compare $LMGP_{CA}$ with $LMGP_{EI}$ and $LMGP_{PI}$. Each example is repeated $20$ times to maintain the robustness.

The former problem is a bi-fidelity example the goal of which is to find the elements of $M_2AX$ compounds that maximize bulk modulus. These compounds are nanolaminate ternary alloys with many advantageous properties of both ceramic and metallic materials. There are three building blocks for the elements of these compounds to take on: an early transition metal $M = \{Sc, T i, V,Cr, Zr, Nb, Mo, H f, T a, W\}$, the main group element $A = \{Al, Si, P, S, Ga, Ge, As,Cd, I n, Sn, T l, Pb\}$, and either carbon or nitrogen $X = \{C, N\}$. The dataset has 224 samples and ten features (three categorical and seven numerical). We began the optimization with $20 ~\text{and} ~10$ high and low-fideity data,respectively with the cost difference of $10$ to $1$.

HOIPs are crystals with the structural formula $ABX_3$. The $B$-site is occupied by metal cations (invariably, Pb, but sometimes Sn, or a mixture of both). The $A$-site cations are either organic or inorganic nature, typically methylammonium (MA), formamidinium (FA), or cesium (Cs). $X$ indicates a possible halide (Cl, Br, and/or I). This dataset has $3$ categorical and $7$ numerical inputs. The first two categorical input are different possible combinations for $X$ and $A$, respectively $X=\{ BrBrBr, BrBrCl, BrBrI, BrClCl, BrClI, BrII, ClClCl, ClClI, ClII, III\}$, $A= \{Cs, FA, MA\}$. The last categorical input denotes the type of the solvent, since these perovskites are usually processed in a solvent blend ($ \{ACE, CH3OH, CHCl3, DMA, DMF, DMSO, ETH, FAM, GBL, H2O, IPA, MCR, NM, NMP,\\ PYR, THTO\}$). 



There are two major challenges associated with studying HOIPs computationally: $(1)$ possible candidate materials differ in composition, $(2)$ the compositional space represents a large combinatorial problem, therefore the computational study of HOIPs has been restricted to expensive density functional theory (DFT) calculations. We use three information sources with the difference in the number of solvents bounded to the lead salt and DFT levels of theory to assess the performance of our proposed cost-aware method on this example with the aim of finding minimum binding energy with lower computational cost. We initialized the model with $15, 20 ~\text{and} ~15$ data from high to low fidelity sources with the cost difference of $15/ 10/ 5$.


Fig.\ref{fig: materila_convergence} demonstrates that $LMGP_{CA}$ found the maximum bulk-modulus faster and at a lower cost than other approaches. Due to the complexity of the problem, $LMGP_{CA}$ has a bit higher initial cost compared to other methods (it required more HF data in the beginning), but its convergence cost is much lower than others. The complexity of the problem and superiority of our proposed model is also obvious in the performance of $LMGP_{EI}$ and $LMGP_{PI}$; despite being SF models that only sample from HF, they were unable to locate the precise ground truth and instead converged to a value that was close to that at a higher cost.

The intricacy of HOIP example is obvious in Fig.\ref{fig: HOIP convergnece} given that neither of the approaches could identify the ground truth. As mentioned in Sec.\ref{sec: BO-LMGP}, MF approaches perform better than SF ones when there is sufficient correlation between the various levels of fidelities. Utilizing the latent map of LMGP, Fig.\ref{fig: fidelity_correlation_HOIP} shows that the rationale behind the underperformance of $LMGP_{CA}$ compared to $LMGP_{EI}$ and $LMGP_{EI}$ is the low correlation between fidelity sources. So, due to the complexity of HOIP problem and low correlation among fidelity sources, neither of the BO approaches could find the optimum with an efficient low number of samples.

Fig.\ref{fig: materila_box-cost} illustrates that $LMGP_{CA}$ and SF approaches perform almost the same in finding the optimum, since $LMGP_{EI}$ and $LMGP_{PI}$ also converged to a value very close to the minimum. However, the superiority of our proposed method comes from its convergence cost. Regarding Fig.\ref{fig: materila_box-iteration}, although $LMGP_{CA}$ took almost the same number of iterations as AF approaches to converge, it managed to sample the most efficient points to find the optimum at the least cost.

Regarding Fig.\ref{fig: HOIP-box-cost} and Fig.\ref{fig: HOIP-box-iter}, considering the low correlation among fidelity sources of HOIP and lower number of iterations taken by $LMGP_{CA}$ compared to other methods, $LMGP_{CA}$ had an acceptable performance in finding the optimum, since it converged to a value close to minimum. This acceptable performance under the existing challenges is an indication of our proposed method's ability in efficient sampling which is also shown in Fig.\ref{fig: error-bar-HOIP}. Regarding this figure, $LMGP_{CA}$ managed to mostly sample from LF sources to reduce the uncertainty of the domain, and only took a few HF samples which largely improved it.


In this paper, we proposed a novel MFCA BO approach by developing cost-aware AFs that consider the biases of LF data and source-dependent sampling costs in addition to balancing exploration and exploitation. Then, the most efficient sample and its corresponding source can be identified through an auxiliary optimization process. The tractability and simplicity of the proposed AFs further reduced the computational cost compared to other AFs, especially look-ahead ones, while preserving accuracy. 

We utilized LMGP as the emulator because it outperforms other existing MF emulators (Fig.\ref{fig: emulator comparison}). This superior performance is attributable to LMGP's capacity for learning the relationship between data sources in a non-linear manifold, which is far more precise and visualizable than the emulators that merely use linear operations. The learned manifold detects the discrepancies and correlations among different fidelity sources which is useful in selecting beneficial fidelity sources. Furthermore, LMGP learns all the fidelity sources (not just HF) accurately and does not need the hierarchy of the fidelities.

We compared our proposed MFCA BO method with two SF and one MF approaches through four numerical and two real-world examples.With the exception of HOIP, $LMGP_{CA}$ outperformed other approaches in terms of both cost and value of convergence in every example in spite of extreme cost difference among data sources.  The main criterion for outperforming of the MF methods compared to SF ones is a significant correlation among fidelity sources to improve the surrogate through fusion. So, our model fails to perform well where there is not enough correlation among fidelity sources which is the case in HOIP example.

We close this section by noting that although our proposed MFCA BO approach is applicable to a wide variety of problems of any dimension and cost difference among fidelity sources, there are still some scenarios that it cannot handle, such as multi-output problems, compound functions and multi-objective problems. We will investigate these cases in our future works. 


